Generalized Resilience and Robust Statistics

Robust statistics traditionally focuses on outliers, or perturbations in total variation distance. However, a dataset could be corrupted in many other ways, such as systematic measurement errors and missing covariates. We generalize the robust statistics approach to consider perturbations under any Wasserstein distance, and show that robust estimation is possible whenever a distribution's population statistics are robust under a certain family of friendly perturbations. This generalizes a property called resilience previously employed in the special case of mean estimation with outliers. We justify the generalized resilience property by showing that it holds under moment or hypercontractive conditions. Even in the total variation case, these subsume conditions in the literature for mean estimation, regression, and covariance estimation; the resulting analysis simplifies and sometimes improves these known results in both population limit and finite-sample rate. Our robust estimators are based on minimum distance (MD) functionals (Donoho and Liu, 1988), which project onto a set of distributions under a discrepancy related to the perturbation. We present two approaches for designing MD estimators with good finite-sample rates: weakening the discrepancy and expanding the set of distributions. We also present connections to Gao et al. (2019)'s recent analysis of generative adversarial networks for robust estimation.

==> finite_sample.tex <==
\section{Finite Sample Algorithms for $\TV$}\label{sec.finite_sample_algorithm_TV}
In Section~\ref{sec.population_limit} we saw that the minimum distance functional defined as 
    \begin{align}
    \label{eq.projection_algo_1}
        q & = \argmin_{q\in \GG} \TV(q,p) \\
    \label{eq.projection_algo_1b}
        \hat \theta &  = \theta^*(q) = \argmin_{\theta \in \Theta} L(q, \theta).
    \end{align}
yields good bounds whenever the modulus of continuity $\modu(\GG, \epsilon)$ is small.
In Sections~\ref{sec.design_G}  we saw how to construct \emph{resilient} sets such 
that the modulus $\modu$ is small, and thus such that the minimum distance functional performs well in infinite samples.
We refer to (\ref{eq.projection_algo_1}) as the projection algorithm because it projects $p$ onto the destination set $\GG$.


Ideally, we would like to turn this infinite-sample algorithm into a finite-sample algorithm 
by substituting $p$ with the empirical distribution $\hat p_n$ in \eqref{eq.projection_algo_1}.
In other words, we would obtain $q$ via
\begin{align}\label{eqn.pluginempirical}
     q = \argmin_{q\in \GG} \TV(q,\hat p_n).
\end{align}
However, in many cases this method fails completely. For example, if $\GG$ only consists of continuous distributions,
then $\TV(q, \hat p_n) = 1$ for all $q\in\GG$, rendering the projection algorithm meaningless. 
In this section, we provide two ways to {fix} the finite sample projection algorithm: 
\begin{enumerate}
    \item \emph{Weaken the discrepancy $\TV$:} one may choose to project under a different function $D (q,\hat{p}_n)$;
    \item \emph{Expand the destination set $\GG$}: one may choose to project to a different set $\mathcal{M}$.
\end{enumerate}

The intuition behind weakening the discrepancy $\TV$ is   too strong such that 
$\TV(p^*, \hat p_n)$ is very large, perhaps a weaker 
related discrepancy $\tTV$ would allow $\tTV(p^*, \hat p_n)$ to be small.
Meanwhile, expanding the destination set $\GG$ seeks to guarantee that there 
is \emph{some} distribution $q\in\GG$ (perhaps not $p^*$ itself) such that $\TV(q, \hat p_n)$ is small 
for the original discrepancy. The general projection algorithm is presented below. 



\begin{algorithm}[H]
\begin{algorithmic}
\State \textbf{Input} 
observed distribution $\hat{p}_n$, discrepancy $D$, destination set $\cM$, optional parameter $\tilde \epsilon$
\If {$\tilde \epsilon$ is given} \\
{\quad
find any $q \in \mathcal{M}$ such that $D(q, \hat{p}_n)\leq \tilde \epsilon$. }
\Else \\
{\quad find $q = \argmin_{q\in \mathcal{M}} {D}(q, \hat{p}_n).$
}
\EndIf
\State \textbf{Output}  $q$.
\end{algorithmic}

 \caption{Projection algorithm $\Pi(\hat{p}_n; D, \mathcal{M})$ or $\Pi(\hat{p}_n; D, \mathcal{M}, \tilde \epsilon)$}\label{alg.general_projection}
\end{algorithm}
Given cost function $L(p, \theta)$, after obtaining $q$ from Algorithm~\ref{alg.general_projection}, 
we output $\hat \theta= \theta^*(q) \triangleq \argmin_{\theta \in \Theta} L(q, \theta)$ as the estimated parameter.

This algorithm is a generalization of the minimum distance functional~\citep{donoho1988automatic}, where we allow the flexibility of choosing  $D$   for the projection function, and 
 $\MM$ for the destination set, and we allow the algorithm to output any $q\in \mathcal{M}$ satisfying $D(q, \hat{p_n})\leq \tilde \epsilon$ if the parameter $\tilde \epsilon$ is given.
We will explore the effects of $D$ 
in this Section and the effects of $\MM$ in Section~\ref{sec.expand}. 


\subsection{Finite-sample algorithm: Weaken the Discrepancy}\label{sec.finite_sample_algorithm_weaken}
In this section we focus on the approach of weakening the discrepancy $\TV$  and keeping the destination set intact ($\cM = \GG$)\footnote{All the argument can be extended to the case of projecting onto $\mathcal{M} = \GG_\downarrow \supset \GG$ when $\GG$ is the generalized resilience set. Here for simplicity we keep $\mathcal{M} = \GG$.}.


We define a family of pseudonorms that is weaker than $\TV$, called  \emph{generalized Kolmogorov--Smirnov distance} $\tTV_\mathcal{H}$,  to avoid the issue of projection under $\TV$:
\begin{align} \label{eqn.ksdistancedefinition}
    \tTV_\mathcal{H}(p, q) \triangleq \sup_{f\in\mathcal{H},  t\in \bR}|\bP_p[f(X)\geq t] - \bP_q[f(X) \geq t]|.
\end{align}
When $X$ is a one-dimensional random variable and $\mathcal{H}$ is the singleton $\{\mathrm{Id}: x \mapsto x\}$, 
we recover the Kolmogorov-Smirnov distance~\cite{massey1951kolmogorov}.
When $\mathcal{H}$ contains all functions, $\tTV_\mathcal{H} = \TV$; otherwise $\tTV_\mathcal{H}$ is weaker than $\TV$ distance: $\tTV_\mathcal{H} \leq \TV$. For any $\mathcal{H}$, $\tTV_\mathcal{H}$ is a pseudometric.  






Assume $p^* \in \GG$ and $\TV(p^*, p) \leq \epsilon$ (oblivious corruption model).
The following result generalizes~\citet{donoho1988automatic} and guarantees good performance of the projection algorithm 
as long as we can bound $\tTV_\mathcal{H}(p, \hat p_n)$ along with the modulus of continuity under $\tTV_{\sH}$.
\begin{proposition}\label{prop.tTV_general}
The projection algorithm $q=\Pi(\hat{p}_n; \tTV_{\mathcal{H}}, \GG)$  satisfies
\begin{align}\label{eqn.tTV_modulus_general}
    L(p^*, \theta^*(q)) \leq  
    \modu(\GG, \tilde\epsilon, \tTV_\mathcal{H}, L) = \sup_{p_1, p_2\in \GG: \tTV_\mathcal{H}(p_1, p_2) \leq \tilde \epsilon} L(p_2, \theta^*(p_1)), 
\end{align} where $\tilde \epsilon = 2\epsilon + 2\tTV_\mathcal{H}(p, \hat p_n)$. 
\end{proposition}

As its proof below shows, the conclusions in Proposition~\ref{prop.tTV_general} remain unchanged if we change the corruption model to 
allow $\tTV_{\sH}$ perturbations instead of $\TV$.
In other words, Proposition~\ref{prop.tTV_general} analyzes the original algorithm under larger corruptions, and we will obtain good finite sample error bounds throughout this section for this more difficult problem. 












\begin{proof}
Since $\tTV_\mathcal{H}$ satisfies triangle inequality, we have 
\begin{align}
    \tTV_\mathcal{H}(q, p^*) & \leq  \tTV_\mathcal{H}(q, \hat p_n) + \tTV_\mathcal{H}(\hat p_n, p^*) \leq 2\tTV_\mathcal{H}(\hat p_n, p^*),
\end{align} 
where the second step is because $\tTV_{\sH}(q, \hat{p}_n)$ is minimizes $\tTV_{\sH}(\cdot, \hat{p}_n)$ over $\GG$. 
Applying the triangle inequality again and $\tTV_\sH(p^*,p)\leq \epsilon$, we obtain
\begin{align}
2\tTV_{\mathcal{H}}(\hat p_n, p^*) \leq 2(\tTV_\mathcal{H}(\hat p_n, p) + \tTV_\mathcal{H}(p, p^*))  \leq 2\epsilon + 2\tTV_\mathcal{H}(p, \hat p_n).
\end{align}
Thus from $p^*, q \in \GG$ and Lemma~\ref{lemma.population_limit},
we know that the error is bounded by $ \modu(\GG, \tilde\epsilon, \tTV_\mathcal{H}, L)$.
\end{proof}


We can bound $\tTV_\mathcal{H}(p, \hat p_n)$ using the following lemma. We defer its proof to Appendix~\ref{Appendix.proof_vcinequality}.
\newcommand{\vc}{\mathsf{vc}}
\begin{lemma}\label{lemma.vcinequality}
Let $\hat{p}_n$ be the empirical distribution of $n$ \iid samples from $p$ and let $\vc(\sH)$ be the VC dimension of the collection of sets $\{\{x \mid f(x)\geq t\} \mid f\in \mathcal{H},t\in \mathbf{R}\}$. Then, each of the following holds with probability at least $1-\delta$:
\begin{align}\label{eqn.vc_inequality}
    \tTV_\mathcal{H}(p,\hat{p}_n) &\leq C^{\mathsf{vc}} \cdot \sqrt{\frac{\mathsf{vc}(\mathcal{H})+\log(1/\delta)}{n} } \text{ for some universal constant $C^{\vc}$}, \\
\label{eqn.dkwtvh}
        \tTV_\mathcal{H}(p,\hat{p}_n) &\leq \sqrt{\frac{\ln(2|\mathcal{H}|/\delta)}{2n}}, \text{ where $|\sH|$ denotes the cardinality of $\sH$.}
    \end{align}
\end{lemma}


Since Lemma~\ref{lemma.vcinequality} bounds $\tTV_{\sH}(p, \hat{p}_n)$, it remains to bound the modulus $\modu(\GG, \epsilon, \tTV_{\sH})$ for some $\sH$ with small VC dimension. 
We show how to do this for different concrete cases below.



\subsubsection*{$\tTV_{\sH}$ projection for mean estimation}
For mean estimation in Example~\ref{example.mean_psi}, we choose $\mathcal{H}$ as
\begin{align}\label{eqn.hlinearnorm}
    \mathcal{H} = \{v^\top X \mid v\in \bR^d\}.
\end{align}
This particular $\tTV_\mathcal{H}$ is also used in~\citet{donoho1982breakdown,donoho1988automatic}.
Intuitively, the reason for choosing this $\sH$ is that linear projections of our data contain all information needed to recover the mean, so perhaps it is enough for distributions to be close only under these projections.

In Section~\ref{sec.design_G},  we controlled the modulus of continuity by using the existence of a midpoint distribution when two distributions are close in $\TV$ (Lemma \ref{lem.G_TV_mean_modulus}). Here we extend it to the mid-point lemma for two 1-dimensional distributions under $\tTV_\mathcal{H}$. %


\begin{lemma}[Midpoint for $\tTV$]
\label{lem.tvt_midpoint} 
Suppose two distributions $p,q$ on the real line satisfy
\begin{align}\label{eqn.tTV_XY}
\sup_{t\in \bR} |\bP_p(X\geq t) - \bP_q(Y\geq t)| \leq \epsilon.
\end{align}

Then one can find some distribution $r$ with $r(A) \leq \frac{p(A)}{1-\epsilon}$ and $r(A) \leq \frac{q(A)}{1-\epsilon}$ for any event $A\in\mathcal{A} = \{X\geq t, X\leq t \mid t\in\bR\}$.
Furthermore, $\sup_{r(A)\leq \frac{p(A)}{1-\epsilon}, \forall A \in\mathcal{A}} |\bE_r[X] - \bE_p[X]| = \sup_{r\leq \frac{p}{1-\epsilon}} |\bE_r[X] - \bE_p[X]|$.
\end{lemma}
\begin{proof}
To guarantee that $r(A) \leq \frac{p(A)}{1-\epsilon}$ and $r(A) \leq \frac{q(A)}{1-\epsilon}$ for any event $A\in\mathcal{A} = \{X\geq t, X\leq t \mid t\in\bR\}$, it is equivalent to the following constraints:
\begin{align*}
    \frac{\max( \bP_p(X\leq t), \bP_q(X\leq t) ) - \epsilon}{1-\epsilon}\leq \bP_r(X\leq t) \leq \frac{\min(\bP_p(X\leq t),\bP_q(X\leq t))}{1-\epsilon}, \forall t\in\bR. 
\end{align*}
Such distribution $r$  exists since it is always true that $ \min(\bP_p(X\leq t),\bP_q(X\leq t)) \geq \max( \bP_p(X\leq t), \bP_q(X\leq t) ) - \epsilon$.

Now it suffices to argue that $\sup_{r(A)\leq \frac{p(A)}{1-\epsilon}, \forall A \in\mathcal{A}} |\bE_r[X] - \bE_p[X]| = \sup_{r\leq \frac{p}{1-\epsilon}} |\bE_r[X] - \bE_p[X]|$. We consider the case when $\bE_r[X] \geq \bE_p[X]$. Then the left-hand side is equivalent to the following constrained optimization problem:
\begin{align}
    \sup_{F} & -\int_{-\infty}^0 F(t)dt + \int_{0}^{+\infty} (1-F(t))dt
    \nonumber \\ 
     s.t. &  \frac{\bP_p(X\leq t)-\epsilon}{1-\epsilon} \leq F(t) \leq \frac{\bP_p(X\leq t)}{1-\epsilon}, F(-\infty) =0, F(+\infty) =1, F:\text{non-decreasing}
\end{align}
One can see that it is maximized at the case when $F(t)$ is minimized everywhere, i.e. $F(t) =  \frac{\bP_p(X\leq t)-\epsilon}{1-\epsilon}, \forall \bP_p(X\leq t)\geq \epsilon, F(t) = 0$ otherwise, which achieves the same supremum when we restrict $r\leq p/(1-\epsilon)$. Similarly when $\bE_r[X]< \bE_p[X]$, the distance is maximized when $F(t)$ is maximized everywhere, which is equivalent to deleting the largest $\epsilon$ mass. This finishes the proof. 


\end{proof}
With this one-dimensional mid-point lemma, the key idea to show modulus of continuity in high dimension is to identify the optimal projected direction and apply the one-dimensional mid-point lemma in that direction.

\subsubsection{Examples and Results}

 For mean estimation, we apply the analysis above to obtain the following:



\begin{theorem}\label{thm.tTV_mean}
Denote $\tilde \epsilon = 2\epsilon + 2C^{\mathsf{vc}}\sqrt{\frac{d+1+\log(1/\delta)}{n}}$, where $C^{\mathsf{vc}}$ is from Lemma~\ref{lemma.vcinequality}. Assume $p^* \in \GG_{\mathsf{mean}}(\rho(\tilde \epsilon), \tilde \epsilon)$. For $\mathcal{H}$ defined in (\ref{eqn.hlinearnorm}), let $q $ denote the output of the projection algorithm $ \Pi(\hat{p}_n; \tTV_{\mathcal{H}}, \GG)$. Then, with probability at least $1-\delta$, 
\begin{align}\label{eqn.finalboundmeanestimation}
    \|\bE_{p^*}[X] - \bE_q[X]\|\leq 2\rho(\tilde \epsilon) = 2\rho\Bigg(2\epsilon + 2C^{\mathsf{vc}}\sqrt{\frac{d+1+\log(1/\delta)}{n}}\Bigg).
\end{align} 
\end{theorem}



\begin{proof}
By Proposition~\ref{prop.tTV_general} it suffices to bound $\tTV_\mathcal{H}(p, \hat p_n)$ and to bound the modulus of continuity for $\GG$ under $\tTV_\mathcal{H}$. 

Since the VC dimension of hyper-planes in $\bR^d$ is $d+1$, it follows from Lemma~\ref{lemma.vcinequality} that $\tTV_\mathcal{H} \leq C^{\mathsf{vc}}\sqrt{\frac{d+1+\log(1/\delta)}{n}}$ with probability at least $1-\delta$. Now we upper bound the modulus, which equals
\begin{align}
    \sup_{p_1, p_2\in \GG_\mathsf{mean}(\rho(\tilde \epsilon),\tilde \epsilon): \tTV_\mathcal{H}(p_1, p_2) \leq \tilde \epsilon}  \|\bE_{p_1}[X] - \bE_{p_2}[X]\|.
\end{align}
The condition that $\tTV_\mathcal{H}(p_1, p_2) \leq \tilde \epsilon$ implies that for any $v\in\bR^d$,  $\|v\|_* = 1$, where $\|\cdot \|_*$ is the dual norm of $ \|\cdot \|$,
\begin{align}
    \sup_{t\in \bR}|\bP_{p_1}[v^\top X\geq t] - \bP_{p_2}[v^\top X \geq t]| \leq \tilde \epsilon.
\end{align}
 


It follows from Lemma~\ref{lem.tvt_midpoint} and  $p_1, p_2\in \GG_\mathsf{mean}(\rho(\tilde \epsilon), \tilde \epsilon)$ that there exist some distribution $r$ with $r(A) \leq \frac{p(A)}{1-\epsilon}$ and $r(A) \leq \frac{q(A)}{1-\epsilon}$ for any event $A\in\mathcal{A} = \{v^\top X\geq t, v^\top X\leq t \mid t\in\bR\}$, and   
\begin{align}
   | \bE_{p_1}[v^\top X]  - \bE_{r}[v^\top X]| \leq \rho(\tilde \epsilon), 
   | \bE_{r}[v^\top X]  - \bE_{p_2}[v^\top X]| \leq \rho(\tilde \epsilon).
\end{align}
This yields $\bE_{p_1}[v^{\top}X] - \bE_{p_2}[v^{\top}X] \leq 2\rho(\tilde \epsilon)$, or 
$v^{\top}(\mu_{p_1} - \mu_{p_2}) \leq 2\rho(\tilde \epsilon)$. Taking the maximum over $\|v\|_* = 1$ yields 
$\|\mu_{p_1} - \mu_{p_2}\| \leq 2\rho(\tilde \epsilon)$, where $\|\cdot \|_*$ is the dual norm of $ \|\cdot \|$.
which shows the modulus is small. The final conclusion follows from Proposition~\ref{prop.tTV_general}. 
\end{proof}



\subsubsection*{Interpretation and Comparison}
If $p^*$ is sub-Gaussian, then $\rho(x) = \Theta(x \sqrt{\log(1/x)})$ and~(\ref{eqn.finalboundmeanestimation}) 
implies an error $O(\epsilon\sqrt{\log(1/\epsilon)})$
when $n \gtrsim \frac{d + \log(1/\delta)}{\epsilon^2}$.
If $p^*$ has bounded covariance, then $\rho(x) = \Theta(\sqrt{x})$ and (\ref{eqn.finalboundmeanestimation}) implies an error of order
    $O(\sqrt{\epsilon})$ when $n \gtrsim \frac{d + \log(1/\delta)}{\epsilon^2}$.

In both cases above, the dependence of $n$ on $\epsilon$ is suboptimal; we improve the sample complexity by another analysis method in Section~\ref{sec.expand}, and defer the detailed discussion to Section~\ref{sec.mean_comparison_discussion}. 






\subsubsection*{$\tTV_{\sH}$ projection for linear regression}
For the linear regression problem in Example~\ref{example.G_TV_linreg}, we design the corresponding $\mathcal{H}$ as
\begin{align}\label{eqn.H_linreg}
\mathcal{H}& = \{(Y - X^\top\theta_1)^2 - (Y - X^\top\theta_2)^2 \mid  \theta_1, \theta_2 \in \bR^d\}.
\end{align}
For linear regression, we need to slightly shrink the resilient set from 
$
    \GG_\downarrow(\rho_1(\tilde \epsilon), \tilde \epsilon)\cap \GG_\uparrow(\rho_1(\tilde \epsilon), \rho_2(\tilde \epsilon), \tilde \epsilon)
$
to 
$
    \GG_\downarrow(\rho_1(\tilde \epsilon), \tilde \epsilon)\cap \GG_\uparrow(2\rho_1(\tilde \epsilon), \rho_2(\tilde \epsilon), \tilde \epsilon).
$
The conditions from Example~\ref{example.G_TV_linreg} still imply that $p^*$ is inside this 
smaller set with appropriate parameters.
The shrinkage comes from the following consideration: 
when using the mid-point lemma, we can only find the mid-point for $p $ and $q$ under the same transform function $f(X)$  while the excess predictive loss in the original $\GG$ requires the mid-point for two different functions.

The following theorem characterizes the performance of $\tTV_{\mathcal{H}}$ projection for linear regression.   We defer the proof to Appendix~\ref{appendix.proof_linreg_tvt}. 
\begin{theorem} \label{thm.linearregressiontvtildeproof}
Denote $\tilde \epsilon =  2\epsilon + 2 C^{\mathsf{vc}}\sqrt{\frac{10d +\log(1/\delta)}{n} }$.
Assume $p^* \in \GG_\downarrow(\rho_1(\tilde \epsilon), \tilde \epsilon)\cap \GG_\uparrow(2\rho_1(\tilde \epsilon), \rho_2(\tilde \epsilon), \tilde \epsilon)$ in Example~\ref{example.G_TV_linreg}. For $\mathcal{H}$ designed in (\ref{eqn.H_linreg}), let $q$ denote the output of the projection algorithm $\Pi(\hat{p}_n; \tTV_{\mathcal{H}}, \GG)$. Then, with probability at least $1-\delta$, 
\begin{align}
    \bE_{p^*}[(Y-X^\top\theta^*(q))^2 - (Y-X^\top\theta^*(p^*))^2]\leq \rho_2(\tilde \epsilon) = \rho_2\Bigg( 2\epsilon + 2 C^{\mathsf{vc}}\sqrt{\frac{10d +\log(1/\delta)}{n} }\Bigg).
\end{align} 
\end{theorem}


\subsubsection*{Interpretation and comparison} 
Combining the above result with the interpretation of Example~\ref{example.G_TV_linreg}, under $k$-hyper-contractivity condition of $X$ and bounded $k$-th moment condition of $Y-X^\top \theta^*(p)$, 
our projection algorithm guarantees the excess predictive loss to be  $O(\epsilon^{2-4/k})$ given $O(d/\epsilon^2)$ samples, while \citet{klivans2018efficient} gives $O(\epsilon^{1-2/k})$ assuming $O(\mathsf{poly}(d^k,1/\epsilon))$ samples. This also matches the dependence on $\epsilon$ with a better dependence on dimension compared to the follow-up work in~\citet{bakshi2020robust}. 

When $X$ and $Z$ are both sub-Gaussian, our dependence on $\epsilon$ is the same as the Gaussian example in~\citet{gao2017robust} up to a log factor while the sample complexity matches~\citet{gao2017robust} exactly. 
\citet{diakonikolas2019efficient} guarantee parameter error $\|\hat \theta - \theta^*\|_2 \lesssim (\epsilon\log(1/\epsilon))^2$ given $O(d/\epsilon^2)$ samples when $X$ is isotropic Gaussian and $Z$ has bounded second moment, which is implied by our analysis by taking the $\psi$ in Example~\ref{example.G_TV_linreg} as exponential function and use it as the generalized resilience set.




\subsubsection*{$\tTV_{\sH}$ projection for second moment estimation}
Let $M_p = \bE_p[XX^{\top}]$. 
For second moment estimation under the loss $L(p,M) = \|I - M_p^{-1/2}M M_p^{-1/2}\|_F$ in Example~\ref{example.G_TV_sec1}, we 
take $\sH$ to be
\begin{align}\label{eqn.H_sec_multiplicative}
    \mathcal{H} & = \{\mathsf{Tr}(A(I - M^{-1/2}XX^{\top}M^{-1/2})) \mid  \|A\|_F\leq 1, M \in \bR^{d\times d} \},
\end{align}
motivated by the dual representation
of $ B(p,M) = \|I - M^{-1/2}M_pM^{-1/2}\|_F$ as the Frobenius norm.


Directly applying mid-point lemma to $f\in\mathcal{H}$ cannot control the modulus since $B(p,M)$ does not satisfy triangle inequality.
Instead, we apply minimax theorem to control the modulus of continuity (general version Lemma~\ref{lemma.minimaxmodulus}). We show the theorem as below and defer the proof to Appendix~\ref{appendix.sec_tvt_proof}. 

\begin{theorem}\label{thm.secondmomenttvtilde}
Denote $\tilde \epsilon = 2\epsilon + 2 C^{\mathsf{vc}} \sqrt{\frac{d^2+1+\log(1/\delta)}{n}}$.  Assume $p^* \in \GG(\rho_1(\tilde \epsilon), \rho_2(\tilde \epsilon),  \tilde \epsilon))$ in Example~\ref{example.G_TV_sec1}. For $\mathcal{H}$ designed in (\ref{eqn.H_sec_multiplicative}), let $q$ denote the output of the projection algorithm $\Pi(\hat{p}_n; \tTV_{\mathcal{H}}, \GG)$. Then, with probability at least $1-\delta$, 
\begin{align}
    \|I  - M_q^{-1/2} M_{p^*}M_q^{-1/2} \|_F \leq \rho_2(\tilde \epsilon) = \rho_2\left (2\epsilon + 2 C^{\mathsf{vc}} \sqrt{\frac{d^2+1+\log(1/\delta)}{n}} \right ).
\end{align}
\end{theorem}



\subsubsection*{Interpretation and Comparison}

\citet{diakonikolas2017being} constructed an algorithm that achieves error $\epsilon \log(1/\epsilon)$ with constant probability given sample size $n \gtrsim \frac{d^2}{\epsilon^2} \mathrm{polylog}(d/\epsilon)$ when the real distribution is Gaussian. We achieve the same error for all resilient distributions given sample size $n\gtrsim \frac{d^2}{\epsilon^2}$.

\subsubsection*{$\tTV$ projection for joint mean and covariance estimation}

Similarly, we can apply the $\tTV$ projection algorithm for joint mean and covariance estimation. We present the theorem as below, and leave the related discussion and proof to Appendix~\ref{appendix.tTV_joint}. Assume the oblivious corruption model of level $\epsilon$. Denote the empirical distribution of observed data as $\hat p_n$. We have the following theorem for Example~\ref{example.G_TV_joint}:
 \begin{theorem}\label{thm.tTV_joint_multiplicative}
Denote $\tilde \epsilon = 2\epsilon + 2C^{\mathsf{vc}}\sqrt{\frac{d+1+\log(1/\delta)}{n}}, \GG = \bigcap_{\epsilon \in[0, 1/2)}\GG_\downarrow(\rho(\epsilon),  \epsilon)$, where $ \GG_\downarrow$ is the same as in Example~\ref{example.G_TV_joint}. Assume $\tilde \epsilon < 1/2$, $p^* \in \GG$ .  For $\mathcal{H} = \{v^\top x \mid v\in\bR^d, \|v\|_2=1\}$, let $q$ denote the output of the projection algorithm $\Pi(\hat{p}_n; \tTV_{\mathcal{H}}, \GG)$ or $\Pi(\hat{p}_n; \tTV_{\mathcal{H}}, \GG, \tilde{\epsilon}/2)$. Then there exist some $C_1$ such that when $\tilde \epsilon \leq C_1$, with probability at least $1-\delta$, 
\begin{align}
     \|\Sigma_{p^*}^{-1/2}(\mu_{p^*} -\mu_q) \|_2 & \lesssim \sqrt{\tilde \epsilon\rho(3\tilde \epsilon)}, \\
    \| I_d - \Sigma_{p^*}^{-1/2}\Sigma_q\Sigma_{p^*}^{-1/2}\|_2 & \lesssim \rho(3\tilde \epsilon).
\end{align}
\end{theorem}
 
\subsubsection{Discussion on the results}\label{subsec.discussion_tTV}

\paragraph*{Not only the minimizer works in MD functional}

We show in Proposition~\ref{prop.any_q_suffices_oblivious}  that instead of looking for the exact projection $ q = \Pi(\hat{p}_n; \tTV_{\mathcal{H}}, \GG)$, all the above results also hold if we simply find some distribution $q=\Pi(\hat{p}_n; \tTV_{\mathcal{H}}, \GG, \tilde \epsilon/2)$ in Algorithm~\ref{alg.general_projection}, i.e. it suffices to find some $q \in \GG$ that is within $\epsilon + f(n, \delta, \mathcal{H})$ $ \tTV_\mathcal{H}$-distance of $\hat p_n$, where $f(n, \delta, \mathcal{H})$ is the $1- \delta$ quantile of $\TV(p, \hat p_n)$, which usually takes the form $C^{\mathsf{vc}}\cdot \sqrt{\frac{\mathsf{vc}(\mathcal{H})+\log(1/\delta)}{n} }$ (Lemma~\ref{lemma.vcinequality}).

\paragraph*{Choice of $\mathcal{H}$ in $\tTV_{\mathcal{H}}$ for general $B$}

In the above examples, we give specific choice of $\mathcal{H}$ for different $\GG$, including $\GG$ for mean estimation, linear regression and second moment estimation under Frobenius norm. We remark that all the choice of $\mathcal{H}$ can be unified by the dual representation of bridge function $B$.
Assume $B(p, \theta)$ is convex in $p$ for all $\theta$ in $\GG(\rho_1, \rho_2, \eta)$, consider the Fenchel-Moreau dual representation~\cite{borwein2010convex} of $B$:
\begin{align*}
    B(p, \theta) = \sup_{f\in\sF_\theta} \bE_p[f(X)] - B^*(f, \theta).
\end{align*}
Here $\sF_\theta = \{f \mid B^*(f,\theta) <\infty\}$. Then we take 
\begin{align}\label{eqn.generaldesignofhusedweaken}
    \mathcal{H}=  \bigcup_{\theta\in \Theta} \sF_\theta.
\end{align}
All the three examples above are taking the $\mathcal{H}$ according to this rule. 
We can also use $\tTV_{\mathcal{H}}$ projection for joint mean and covariance estimation; the detailed discussion is deferred to Appendix~\ref{appendix.tTV_joint}, where we adopt a different method other than mean cross lemma to show the modulus, and discuss the recovery under two different choices of the loss $L$. For multiplicative cost (Theorem~\ref{thm.tTV_joint_multiplicative}), our results get the same population limit as~\citet{kothari2017outlier}
while improving the sample complexity's dependence on dimension from $O((d\log(d))^k/2)$ to $O(d)$. For cost under 2-norm (Theorem~\ref{thm.tTV_joint_correct}), our results generalize the result in \citet{gao2019generative} from Gaussians to a non-parametric set with a necessary sacrifice of a log factor. 

\paragraph*{Performance guarantee for adaptive corruption model}

So far we only focus on the performance guarantee for oblivious corruption model. In fact, all the above results also hold for adaptive corruption model. We only need to substitute the term $\tilde \epsilon = 2\epsilon + 2 C^{\mathsf{vc}} \sqrt{\frac{\mathsf{vc}(\mathcal{H})+\log(1/\delta)}{n}}$ in the results with $\tilde \epsilon = 2(\sqrt{\epsilon}+\sqrt{\frac{\log(1/\delta)}{n}})^2   + 2 C^{\mathsf{vc}} \sqrt{\frac{\mathsf{vc}(\mathcal{H})+\log(1/\delta)}{n}}$. The results can be seen from a combination of Theorem~\ref{thm.admissible-1-adaptive} for analysis technique and Lemma~\ref{lem.coupling_TV} for the upper bound on $\TV(\hat p_n, \hat p_n^*)$.  The difference in analysis is sketched in Theorem~\ref{thm.admissible-1} and Theorem~\ref{thm.admissible-1-adaptive}.



\subsection{Finite Sample Algorithms - Expand Destination Set $\mathcal{M}$}\label{sec.expand}








Besides weakening the distance $  \TV$, an alternative way to rescue the projection algorithm 
is to ensure that the destination set $\cM$ is {large enough}. 
In this section, we assume the corruption model is either oblivious corruption (Definition~\ref{def.obliviouscorruption}) or adaptive corruption (Definition~\ref{def.adaptivecont}) of level $\epsilon$, and denote $\hat p_n$ as the corrupted empirical distribution and $\hat{p}_n^*$ as the empirical distribution sampled from the clean population distribution $p^*$.  %







We will focus on mean estimation because it is well-studied, but our analysis 
strategy applies more generally.  
Interestingly, all the results in this section apply to both $\TV$ and $\tTV$ projection. For $\TV$ projection, the existing filtering and convex programming approaches can be viewed as obtaining one solution of our projection; for $\tTV_\mathcal{H}$ projection, our results provide new bounds for the algorithm in Section~\ref{sec.finite_sample_algorithm_weaken}. 
We summarize the idea of analyzing $\TV$ projection in Figure~\ref{fig.projection_illustration}. The key difference of this approach compared to distance weakening is that we no longer search for the population distribution $p^*$ in projection; we instead search for the empirical distribution $\hat{p}_n^*$ in projection. Concretely, for projection onto $\MM$ to work well, the following three properties suffice:
\begin{itemize}
\item $\MM$ is large enough: $\hat p_n^* \in \MM$ with high probability. 
\item The empirical loss $L(\hat p_n^*, \theta)$ is a good approximation to the population loss $L(p^*, \theta)$.
\item The modulus is still bounded:  $\min_{p, q \in \MM : \TV(p, q) \leq 2\epsilon} L(p, \theta^*(q))$ is small.
\end{itemize}

In fact, we only need $\hat p_n^*$ to be \emph{near} $\cM$ with high probability, as long as there exists some $\hat p' \in \MM$ 
such that $\TV(\hat p', \hat p_n^*)$ is small and $L(\hat p', \theta)$ is a good approximation to $L(p^*, \theta)$. Moreover, we get stronger bounds when this $\hat p'$ (or $\hat p_n^*$ itself) lies in some smaller set $\GG' \subset \cM$. This is formalized in the following proposition: 


\begin{proposition}
\label{prop.expand_sufficient}
For a set $\GG' \subset \MM$, define the generalized modulus of continuity as 
\begin{equation}
\modu(\GG', \MM, \epsilon) \eqdef \min_{p \in \GG', q \in \MM : \TV(p, q) \leq \epsilon} L(p, \theta^*(q)).
\end{equation}
Assume $\TV(\hat p', \hat p_n^*)\leq \epsilon_1$  with probability at least $1-\delta$ and $\hat p' \in \GG'$ with probability at least $1-\delta$.
Then the minimum distance functional projecting under $\TV$ onto $\MM$ has empirical error 
$L(\hat p', \hat{\theta})$ at most $\modu(\GG', \MM, \tilde \epsilon)$ with probability at least 
$1 - 3\delta$, where $\tilde \epsilon =2(\sqrt{\epsilon}+\sqrt{\frac{\log(1/\delta)}{2n}})^2+2\epsilon_1$.
\end{proposition}

\begin{proof}
From Lemma~\ref{lem.coupling_TV}, we know that with probability at least $1-\delta$, $\TV(\hat p_n^*, \hat p_n)\leq (\sqrt{\epsilon}+\sqrt{\frac{\log(1/\delta)}{2n}})^2$. Thus by triangle inequality, $\TV(\hat p_n, \hat p')\leq \epsilon_1 + (\sqrt{\epsilon}+\sqrt{\frac{\log(1/\delta)}{2n}})^2 = \tilde \epsilon/2$ with probability at least $1-2\delta$.
If $\hat p'$ lies in $\GG'$, then since $\GG' \subset \MM$ we know that $\hat{p}_n$ has distance 
at most $\tilde \epsilon/2$ from $\MM$, and so the projected distribution $q$ satisfies $\TV(q, \hat{p}_n) \leq \tilde \epsilon/2$ 
and hence $\TV(q, \hat p') \leq \tilde \epsilon$. It follows from the definition that 
$L(\hat p', \hat{\theta}) = L(\hat p', \theta^*(q)) \leq \modu(\GG', \MM, \tilde \epsilon)$.
\end{proof}

To employ Proposition~\ref{prop.expand_sufficient}, we construct $\MM$ and $\GG'$ such that 
the generalized modulus is small, then exhibit some $\hat{p}' \in \GG'$ that is close to 
$\hat{p}_n^*$. Often $\hat{p}'$ will just be $\hat{p}_n^*$, but sometimes it is a perturbed 
version of $\hat{p}_n^*$ that deletes heavy-tailed ``bad'' events. 

\begin{figure}[!htbp]
\centering
\begin{tikzpicture}
    \draw [opacity=1, very thick, fill=red!50, draw= red!50!black](2.4, 0.0) {ellipse (2cm and 1cm)};
     \draw [opacity=0.6,  very thick, fill= cyan!20, draw= cyan!20!black](2.0, 1.0) {ellipse (3cm and 2.5cm)};
      \draw [opacity=0.4, fill= yellow!20, draw= yellow!20!black](2.5, 1.5) {ellipse (4.5cm and 3.2 cm)};
     \draw  [](3.3, -0.5) node {$p^*\in\GG$};
     \draw  [](1.3, 0) node {\Large $\GG$};
     \draw  [](0.3, 1.8) node {\Large $\GG'$};
     \draw  [](-0.6, 3.5) node {\Large $\cM$};
       \draw [radius=1.5pt,fill](3.4, -0.23) circle;
     \draw  [](3.35, 2.42) node {$\hat p'\in\GG'$};
      \draw [radius=1.5pt,fill](3.5,2.85) circle;
     \draw  [](2.6,5.2) node {$\hat p_n^*$};
      \draw [radius=1.5pt,fill](2.8, 4.85) circle;
    \draw  [](4.51, 4.67) node {$q\in\cM$};
      \draw [radius=1.5pt,fill](4.5,4.3) circle;
     \draw  [](9,4.5) node {Observed distribution $\hat p_n$};
      \draw [radius=1.5pt,fill] (7.2, 4.0) circle;
    \draw (7.2, 4.0) edge[->] node[below, rotate=48,yshift=-1.5]{{\scriptsize $ \tTV_\mathcal{H}\lesssim \epsilon + \sqrt{\mathsf{vc}(\mathcal{H})/n}$, $\TV$ large}} (3.4, -0.23);
    \draw (7.2, 4.0) edge[->] node[above, rotate=16, xshift=-0.5]{{\scriptsize $\tTV_\sH\leq  \TV\lesssim \epsilon + 1/n$}} (3.5,2.85); 
    \draw (7.2, 4.0) edge[->] node[above, rotate=-8]{{\scriptsize projection}} (4.56,4.3);
     \draw (2.8, 4.85) edge[->] node[below, rotate=-70]{{\scriptsize $\TV$ small}} (3.45,2.9);
\end{tikzpicture}
\caption{
Illustration of projection algorithm. By perturbing $\hat p_n^*$ to $\hat p'$ a small amount ($\TV(\hat p_n^*, \hat p')\lesssim \epsilon + 1/n$) under $\TV$, we can ensure $\hat p' \in \GG'$ and control $\TV(\hat p_n, \hat p')$ simultaneously. Thus projecting $\hat p_n$ onto a larger set $\cM$ can guarantee $ \tTV_\sH(q, \hat p_n)\leq \TV(q, \hat p_n)\lesssim \epsilon+1/n$. In contrast, projecting onto the original $\GG$ (as Section~\ref{sec.finite_sample_algorithm_weaken}) can only guarantee $\tTV_\mathcal{H}(q, \hat p_n)\lesssim \epsilon+\sqrt{\mathsf{vc}(\mathcal{H})/n}$, which gives sub-optimal sample complexity in many cases.}
\label{fig.projection_illustration}
\end{figure}












The key difficulty in analysis is that the empirical distribution $\hat p_n^*$ may not inherit the good properties of $p^*$, e.g.~the empirical distribution of an isotropic Gaussian distribution does not have constant $k$-th moment unless the sample size $n \gg d^{k/2}$ for constant $k$. Additionally, when $k = 2$, even if the original distribution has bounded Euclidean norm $\sqrt{d}$, its empirical distribution with $d$ samples is not resilient with the right scale of $\rho = O(\sqrt{\eta})$.
We discussed this in Appendix~\ref{sec.negativeresultresilient}.



























Since we cannot hope to establish properties like bounded $k$th moments for $\hat p_n^*$, we instead rely on three main techniques 
to control some other properties of $\hat p_n^*$ or $\hat p'$:
union bound, moment linearization, and perturbing $\hat p_n^*$ to $\hat p'$.

\subsubsection*{Union bound}
Our first observation is that even if $\GG$ is small, we can take $\MM$ to be the family of resilient 
distributions while maintaining similarly small modulus. 
Thus we only need $\hat{p}_n^*$ to be {resilient},
which is easier to satisfy than e.g.~bounded moments or sub-Gaussianity.
For distributions with moment generating functions, a union bound leads to the following typical result~(Lemma~\ref{lem.subgaussian_empirical_resilience}): if $p^*$ is sub-Gaussian with parameter $\sigma$, then for any fixed $\eta$, the empirical distribution $\hat p_n^*$ 
is $(\rho, \eta)$-resilient with probability $1-\delta$, for $\rho = O(\sigma (\sqrt{\eta \frac{d+\log(1/\delta)}{n}} + \eta \sqrt{\log(1/\eta)}))$, which gives tighter bound for resilience paramter than~\citet[Lemma  4.4]{diakonikolas2019robust}. 
We thus obtain:
\begin{theorem}[Sub-Gaussian]\label{thm.general_subgaussian_tv_projection}
Denote $\tilde \epsilon = 2(\sqrt{\epsilon} + \sqrt{\frac{\log(1/\delta)}{2n}})^2$.
There exist some constants $C_1, C_2$ such that the following statement is true. Take $\GG$ as family of sub-Gaussian with parameter $\sigma$ and $\cM$ as resilient set, i.e.
\begin{align}
    \GG & =  \bigg\{ p \mid \sup_{v\in\bR^d, \|v\|_2=1} \bE_p\bigg[\exp\bigg(\left( \frac{|v^{\top}(X-\bE_p[X])|}{\sigma}\right)^2\bigg) \bigg] \leq  2 \bigg\},\\
  \cM & = \GG_{\mathsf{mean}}\bigg( C_1\sigma\cdot \bigg(\epsilon \sqrt{\log(1/\epsilon)} + \sqrt{ \frac{d+\log(1/\delta)}{n}}\bigg) , \tilde \epsilon \bigg),
\end{align}
where $\GG_{\mathsf{mean}}$ is defined in~\eqref{eqn.oldresilience}.  If $p^*\in\GG$ and $\tilde \epsilon\leq 1/2$,
then the projection $q = \Pi(\hat p_n; \TV / \tTV_\mathcal{H}, \cM)$ of $\hat{p}_n$ onto $\MM$ satisfies:
\begin{align}
 \|\bE_{p^*}[X]- \bE_q[X] \|_2 & \leq   C_2\sigma \cdot \bigg(\epsilon \sqrt{\log(1/\epsilon)} + \sqrt{\frac{d+\log(1/\delta)}{n}} \bigg)
\end{align}
 with probability at least $1-3\delta$. Moreover, 
this bound holds for any $q \in \MM$ within $\TV$ (or $\tTV$) distance $\tilde \eps/2$ of $\hat{p}_n$.

\end{theorem}
The proof is deferred to Appendix~\ref{proof.general_subgaussian_tv_projection}. 

\subsubsection*{Linearized moment} The above technique only applies to the case when the population distribution has a moment generating function, because it requires union bounding over exponentially many events. If instead we only have bounded $k$th moments, we need a different 
approach. Although $\hat p_n^*$ does not have small $k$-th moment with less than $d^{k/2}$ samples, 
our key insight is that we can bound a certain \emph{linearized} $k$-th moment with only $\Theta(d)$ samples, which is {sufficient} to ensure {resilience} (see Lemma~\ref{lem.empirical_psi_resilient} for a rigorous statement and extension to any Orlicz norm). 
For instance, if $p^*$ has $4$th moments bounded by $\sigma^4$ then we will bound $\sup_{\|v\|_2 \leq 1} \bE_{\hat p_n^*}[\psi(|v^{\top}X|)]$, 
where $\psi(x)$ is the smallest convex function on $[0,\infty)$ that coincides with $x^4$ when $0\leq x\leq 4\sigma$ when $n=d$.   

 
Taking $\cM$ to be the set of resilient distributions as before, we obtain:
\begin{theorem}[Bounded $k$-th moment]\label{thm.general_kth_tv_projection}
Denote $\tilde \epsilon = 2(\sqrt{\epsilon} + \sqrt{\frac{\log(1/\delta)}{2n}})^2$.
There exist some constants $C_1, C_2$ such that the following statement is true.
Take $\GG$ as bounded $k$-th moment set for $k\geq 2$ and $\cM$ as resilient set, i.e.
\begin{align}
    \GG & =  \{ p \mid \sup_{v\in\bR^d, \|v\|_2=1} \bE_p[ |v^{\top}(X-\bE_p[X])|^k] \leq  \sigma^k \} \\
  \cM & =  \GG_{\mathsf{mean}}\bigg({C_1k\sigma}\bigg(\frac{\epsilon^{1-1/k}}{\delta^{1/k}}  + \frac{1}{\delta} \sqrt{\frac{d}{n}}\bigg),  \tilde \epsilon \bigg),
\end{align}
If $p^*\in\GG$ and $\tilde \epsilon \leq 1/2$, 
then the projection $q = \Pi(\hat p_n; \TV / \tTV_\mathcal{H}, \cM)$ of $\hat{p}_n$ onto $\MM$ satisfies: 
\begin{align}
    \|\bE_{p^*}[X] - \bE_q[X]\|_2 & \leq  C_2k\sigma\cdot\left(\frac{\epsilon^{1-1/k}}{\delta^{1/k}} +\frac{1}{\delta}\sqrt{\frac{d}{n}}\right)
\end{align}
with probability at least $1-4\delta$.  Moreover, 
this bound holds for any $q \in \MM$ within $\TV$ (or $\tTV$) distance $\tilde \eps/2$ of $\hat{p}_n$.
\end{theorem}


The proof is deferred to Appendix~\ref{proof.general_kth_tv_projection}. \citet{steinhardt2018resilience}
presented an analysis for the same projection algorithm that requires $d^{3/2}$ samples, which our result improves to $d$. 

\subsubsection*{Perturb $\hat p_n^*$ to $\hat p'$} If $p^*$ has covariance operator norm bounded by $\sigma$, then in general with even $d\log d$ samples one cannot guarantee that $\hat p_n^*$ has covariance with operator norm $O(\sigma)$. However, it was realized in~\citet{steinhardt2017resilience} that one may construct another distribution $\hat p'$ with $\TV(\hat p_n^*, \hat p')\lesssim \epsilon$ such that $\hat p'$ has covariance bounded by $O(\sigma)$ given $d\log d$ samples.
Thus instead of checking the empirical distribution $\hat p_n^* \in\GG'$, we can construct some $\hat p' \in \GG'$ such that $\TV(\hat p_n^*, \hat p' ) \lesssim \epsilon$. 
    
This allows us to take $\cM$ to be the set of bounded covariance distributions instead of all resilient distributions; 
the advantage of this is that there are 
computationally efficient algorithms that approximately solve 
the projection in some cases~\cite{diakonikolas2017being, diakonikolas2019efficient}. 

    
    This motivates us to consider mean estimation for bounded $k$-th moment distribution with identity covariance. The identity covariance assumption allows us to take $\cM$ to be the set of bounded covariance distributions, which we believe admits an efficient projection 
algorithm analogous to that of \citet{diakonikolas2017being} for isotropic sub-Gaussians.
    The statistical analysis requires the simultaneous application of the {linearized moment} and {perturbation} techniques described above, as well as a generalized modulus result~(Lemma~\ref{lem.empirical_identity_cov_modulus}). We obtain:
    



\begin{theorem}[Bounded $k$-th moment and identity covariance]\label{thm.projection_kth_moment_identity_covariance}
Denote
$\tilde \epsilon = 4(\sqrt{\epsilon + \frac{\log(1/\delta)}{n}} + \sqrt{\frac{\log(1/\delta)}{2n}})^2$.
Take $\GG$ to be the set of isotropic distributions with bounded $k$-th moment, $k\geq 2$, and $\MM$ to be the set of bounded covariance distributions:
\begin{align}
    \mathcal{G} &= \{p \mid \mathbb{E}_p[(X-\mu_p)(X-\mu_p)^{\top}] = I_d,  \sup_{v\in \bR^d, \|v\|_2 = 1} \bE_p[ |v^{\top}(X - \mu_p)|^k] \leq \sigma^k \},\\
    \mathcal{M} &= \{p \mid  \|\bE_p[(X-\mu_p)(X-\mu_p)^\top] \|_2 \leq 1+ f(n, d, \epsilon, \delta, \sigma)\}.
\end{align}
If $p^*\in\GG$ and $\tilde \epsilon < 1/2$, then there exists some $f(n, d, \epsilon, \delta, \sigma)$ such that the projection $q = \Pi(\hat p_n; \TV / \tTV_\mathcal{H}, \cM)$ of $\hat{p}_n$ onto $\MM$ satisfies
\begin{align}
     \|\mu_{p^*}-\mu_q\|_2 & =   O\left(k\sigma\cdot \left(\frac{ \epsilon^{1-1/k}}{\delta^{1/k}} + \frac{1}{\delta}\sqrt{\frac{d\log(d)}{n}}\right) \right)
\end{align}
with probability at least $1-8\delta$. Moreover,
this bound holds for any $q \in \MM$ within $\TV$ (or $\tTV$) distance $\tilde \eps/2$ of $\hat{p}_n$.
\end{theorem}

The proof is deferred to Appendix~\ref{proof.bounded_kth_identity}. When $\delta$ is constant and $n$ goes to infinity, this bound recovers $O(\epsilon^{1-1/k})$, which is the population limit for bounded $k$-th moment distributions. It also guarantees sample complexity of $O(d\log(d)/\epsilon^{2-2/k})$.


The general framework of this analysis approach  is summarized in Theorem~\ref{thm.admissible-2}, where we analyze the projection algorithm for general $D$, $L$, and $\GG$. 









\subsection{Interpretation and Comparison for Mean Estimation}\label{sec.mean_comparison_discussion}

To contrast the approaches in Sections~\ref{sec.finite_sample_algorithm_weaken} and \ref{sec.expand}, here we compare their implied 
bounds for robust mean estimation (Table~\ref{tab.projection_summary}) and also discuss related literature.
\begin{table}[H]
\hskip-0.9cm
\begin{tabular}{|c|c|c|c|}\hline 
 $\GG$ & $\cM$ & $D$ & $\|\mu_{p^*}-\mu_q\|_2 $ \\
 \hline
 $\GG_{\mathsf{mean}}$ & $\GG_{\mathsf{mean}}$ & $\tTV$ & $\rho(2\epsilon + 2C^{\mathsf{vc}}\sqrt{\frac{d+ 1+\log(1/\delta)}{n}})$ [Theorem~\ref{thm.tTV_mean}]  \\
  sub-Gaussian & $\GG_{\mathsf{mean}}$ & $\TV$ or $\tTV$ & $\epsilon\sqrt{\log(1/\epsilon)} + \sqrt{\frac{d+\log(1/\delta)}{n}} $ [Theorem~\ref{thm.general_subgaussian_tv_projection}]\\
 bdd $k$-th moment ($k\geq 2$) &  $\GG_{\mathsf{mean}} $ &  $\TV$ or $\tTV$ & $\frac{\epsilon^{1-1/k}}{\delta^{1/k}} +\frac{1}{\delta}\sqrt{\frac{d}{n}}$ 
 [Theorem~\ref{thm.general_kth_tv_projection}]\\
 bdd cov  &  bdd cov &  $\TV$ or $\tTV$ & $\sqrt{ \epsilon} +\sqrt{\frac{d\log(d/\delta)}{n}}$ [Theorem~\ref{thm.projection_bounded_covariance}] \\
 bdd $k$-th moment ($k>2$) + $I_d$   &  bdd cov  & $\TV$ or $\tTV$ & $\frac{ \epsilon^{1-1/k}}{\delta^{1/k}} + \frac{1}{\delta}\sqrt{\frac{d\log(d)}{n}}$  [Theorem~\ref{thm.projection_kth_moment_identity_covariance}] \\
 \hline
\end{tabular}
\caption{Summary of results for generalized projection algorithm
assuming $p^*\in\GG$. Here `bdd' is short for `bounded'. }
\label{tab.projection_summary}
\end{table}




\subsubsection*{Interpretation and comparison for $\tTV_\mathcal{H}$ projection algorithm}


If $p^*$ is sub-Gaussian, analysis in Theorem~\ref{thm.tTV_mean} 
implies an error $O(\epsilon\sqrt{\log(1/\epsilon)})$
when $n \gtrsim \frac{d + \log(1/\delta)}{\epsilon^2}$, while  analysis 
in Theorem~\ref{thm.general_subgaussian_tv_projection} shows that the same algorithm actually only  requires $n \gtrsim \frac{d + \log(1/\delta)}{\epsilon^2\log(1/\epsilon)}$, which is optimal. Here 
Theorem~\ref{thm.general_subgaussian_tv_projection} is not explicitly stated in the literature but should be well known among experts. We are also able to generalize it to all distributions with moment generating functions by Lemma~\ref{lem.subgaussian_empirical_resilience}, which provides better bound than~\citet[Lemma  4.4]{diakonikolas2019robust} for sub-Gaussian case.

If $p^*$ has bounded covariance, then Theorem~\ref{thm.tTV_mean} implies an error of order $O(\sqrt{\epsilon})$ when $n \gtrsim \frac{d + \log(1/\delta)}{\epsilon^2}$.
This dependence of $n$ on $\epsilon$ is sub-optimal; inspired by~\citet{prasad2019unified}, our Theorem~\ref{thm.projection_bounded_covariance} shows that the same $\tTV_\mathcal{H}$ projection algorithm reaches $O(\sqrt{\epsilon})$ error when $n \gtrsim \frac{d\log(d/\delta)}{\epsilon}$, 
    which has better dependence of $n$ on $\epsilon$ but worse dependence on $d$.
    
    When $\epsilon = 0$, the current analysis in Theorem~\ref{thm.tTV_mean} for projecting under resilient set
    yields an error of $O((\frac{d+\log(1/\delta)}{n})^{1/4})$ error, and our Theorem~\ref{thm.projection_bounded_covariance} for projecting under bounded covariance set
    gives $O((\frac{d\log(d/\delta)}{n})^{1/2})$,  while median-of-means tournament method~\cite{lugosi2019sub} can achieve $O((\frac{d+\log(1/\delta)}{n})^{1/2})$. In the follow-up work~\cite{diakonikolas2020outlier}, it is shown that the exact sub-Gaussian rate can be achieved by combining the bucket means in median-of-means and $\TV$ projection algorithm, while without the combination one might lose a logarithmic factor. %




\subsubsection*{Interpretation and comparison for $\TV$ projection algorithm}

For  $k$-th moment bounded distributions, 
the \emph{linearized moment} approach~(Lemma~\ref{lem.empirical_psi_resilient}) and Theorem~\ref{thm.general_kth_tv_projection} are new, and prior to our work~\citet{steinhardt2018robust} shows that   projection onto resilient set under $\TV$ distance  works for $k$-th moment bounded distributions with $d^{3/2}$ samples. \citet{prasad2019unified} used the approach of reducing high-dimensional mean estimation to one dimensional to achieve error $\epsilon^{1-1/k} + \sqrt{\frac{d+\log(1/\delta)}{n}}$, while we generalize it to all distributions with bounded Orlicz norms~(Corollary~\ref{cor.kthmomentreduceapproach}) with the one dimensional mean estimator taken as our projection estimator. Theorem~\ref{thm.projection_kth_moment_identity_covariance} presents the first guarantee for potentially efficient mean estimation algorithm of bounded $k$-th moment isotropic distributions with sample complexity $O(d\log d)$. It was shown in the literature that for sub-Gaussian distributions with identity covariance~\cite{diakonikolas2018robustly, diakonikolas2018learning, cheng2019high, cheng2019faster}, one can also choose $\cM$ to be the bounded covariance set to achieve efficient computation and near-optimal statistical rate,



The flexibility of only needing to find some $q \in \MM$ with $\TV(q, \hat p_n) \leq \epsilon$ is useful for efficient algorithms. Indeed, many filtering and convex programming algorithms in the literature~\citet{diakonikolas2018robustly, diakonikolas2018learning, cheng2019high, cheng2019faster} can be interpreted as finding \emph{some} distribution $q \in \MM$, so that our analysis below leads to sample complexity bounds for those and similar algorithms. Usually these efficient algorithms are trying to find $q$ among \emph{deleted} versions of $\hat p_n$, hence even after exhaustive search it is not guaranteed to find the $\hat p'$ {(or} $\hat p_n^*) \in \GG'$ since some of the samples might be already deleted. Hence, one additional step in analyzing the statistical properties of these efficient algorithms is to use our Lemma~\ref{lem.Wf_orlicz_closed} and Lemma~\ref{lem.resilience_closed}, which show that any Orlicz norm bounded set and resilient set are approximately closed under deletion. Thus as long as $\GG'$ is of these types, any deleted version of $\hat p'$ or $\hat p_n^*$ would approximately share the same properties as $\hat p'$ or $\hat p_n^*$. 


However, some filtering algorithms in the literature may not be cast as a projection 
algorithm; for instance in~\citet{diakonikolas2018robustly}, one is required to follow a particular path of deleting $\hat p_n$ to ensure that for each filter step one deletes way more bad points than good points, and the filter there only works under the Huber additive corruption model but not $\TV$ corruption.  






 



==> finite_sample_w1.tex <==
\section{Finite Sample Algorithm for $W_1$}\label{sec.finite_sample_w1}

In this section, we design finite sample algorithms for robust estimation under $W_1$ perturbations.  Throughout the section, we assume that $\hat p_n$ follows oblivious corruption model (Definition~\ref{def.obliviouscorruption}) of level $\epsilon$ under $W_1$ perturbation. It can also be extended to the adaptive corruption model using Theorem~\ref{thm.admissible-1-adaptive}. 

Similar to the issue of $\TV(p, \hat p_n)$ discussed in Section~\ref{sec.finite_sample_algorithm_TV}, in general $W_{c, k}(p, \hat p_n)$ converges to zero slowly even when $p$ is well behaved; for instance,  
$\mathbb{E}[W_1(p, \hat p_n)] \gtrsim_p n^{-1/d}$ for 
any measure $p$ that is absolutely continuous with respect to the Lebesgue measure on $\bR^d$ \citep{dudley1969speed}.
As Section~\ref{sec.finite_sample_algorithm_weaken}, we therefore weaken $W_1$ to a distance $\tW_1$ to achieve better finite sample performance. 


\subsection{Second Moment Estimation: Design of $\tW_1$}
We first introduce our design of $\tW_1$ for second moment estimation. 
In below analysis we assume an oblivious corruption model (Definition~\ref{def.obliviouscorruption}), i.e. $\TV(p^*, p)\leq \epsilon$ and we observe an empirical distribution of $p$. But our results also apply directly to adaptive corruption model (Definition~\ref{def.adaptivecont}) as $\TV$ case, which is shown  from a combination of Theorem~\ref{thm.admissible-1-adaptive} for analysis technique and Lemma~\ref{lem.coupling} for the upper bound on $W_1(\hat p_n, \hat p_n^*)$.

Recall the dual representation of $W_1$:
\begin{align}
    W_1(p, q) = \sup_{u\in \mathcal{U}}  \bE_p[u(X)] - \bE_q[u(X)] ,
\end{align}
where $\mathcal{U} = \{u: \bR^d \mapsto \bR \mid |u(x) - u(y)| \leq \|x-y \|\}$ is the set of all
$1$-Lipschitz functions.

To design the weakened distance $\tW_1(p, q)$, we take the supremum over a smaller set. Let $\sU'$ be the set of all 
$1$-Lipschitz linear or rectified linear functions:
\begin{align}
\mathcal{U}' = \{\max(0, v^{\top}x-a) \mid v\in \bR^d, \|v\|\leq 1, a\in\bR \} \cup \{v^{\top}x \mid v \in \bR^d, \|v\|\leq 1\}.
\end{align} 
Since all functions in $\mathcal{U}'$ are Lipschitz-1, $\mathcal{U}' \subset \mathcal{U}$, and we define $\tW_1$ as follows:
\begin{align}
\label{eqn.tw_def}
    \tW_1(p, q) & = \sup_{u \in \mathcal{U}'} \left|\bE_p[u(X)] - \bE_q[u(X)] \right|.
\end{align}
Similarly to Proposition~\ref{prop.tTV_general}, the key to analyzing $\tW_1(p, q)$ is to control (i) $\tW_1(p, \hat p_n)$ and (ii) the modulus of continuity for $\GG^{W_1}$ under $\tW_1$. 

We first use the following lemma to bound the statistical error $\tW_1(p, \hat p_n)$:

\begin{lemma}\label{lem.tW_1_empirical_to_population}
Assume $W_1(p^*, p)\leq \epsilon$ and for some Orlicz function $\psi$, $p^*$ satisfies 
\begin{align}
   \sup_{v\in\bR^d, \|v\|_2=1} \bE_{p^*}[\psi(|v^\top(X-\mu_{p^*})|/\kappa)] \leq 1, \\
    \|\bE_{p^*}[(X-\mu_{p^*})(X-\mu_{p^*})^\top]\|_2\leq \sigma^2.
\end{align}
Then for $\tW_1$ defined in (\ref{eqn.tw_def}), we have \begin{align}
    \bE_{p}[\tW_1(p, \hat p_n)]\leq 2\epsilon + 8\sigma \sqrt{\frac{d}{n}}+\frac{3\kappa \psi^{-1}(\sqrt{n})}{\sqrt{n}}.
\end{align}
\end{lemma}

The proof is deferred to Appendix~\ref{proof.tW_1_empirical_to_population}. Compared to the lower bound  $\bE[W_1(p, \hat p_n)]\gtrsim n^{-1/d}$, the upper bound for $\tW_1$ reduces the  sample complexity from exponential in $d$ to polynomial in $d$. 


To bound the modulus of continuity, we establish a 
mean cross lemma showing that $p$ and $q$ have friendly perturbations $r_p$ and $r_q$ with 
$\bE_{r_q}[f(X)] \leq \bE_{r_p}[f(X)]$ (cf.~Lemma~\ref{lem.tvt_cross_mean}).
In Lemma~\ref{lem.tvt_cross_mean} for $\tTV$, we established the mean crossing property 
by showing that $r_p$ stochastically dominated $r_q$; for $\tW_1$ we will instead 
show that $r_p$ dominates $r_q$ in the convex order, which establishes 
mean crossing for convex functions $f$:



\begin{figure}[!htp]
    \centering
   \begin{tikzpicture}[
  implies/.style={double,double equal sign distance,-implies},
  scale=0.9,
]
\begin{axis}[
  no markers, domain=0:8, samples=50,
  axis lines*=left,
  every axis y label/.style={at=(current axis.above origin),anchor=south},
  every axis x label/.style={at=(current axis.right of origin),anchor=west},
  height=5cm, width=12cm,
  xtick=\empty, ytick=\empty,
  enlargelimits=false, clip=false, axis on top,
  axis line style = thick,
  grid = major
  ]
  \addplot+[opacity=0.8,very thick,fill=cyan!50, draw=cyan!50!black, domain=0:8] {gauss(3.6,0.6,1)} \closedcycle;
  \addplot+[opacity=0.7,very thick,fill=red!30, draw=none, domain=4.3:8]
  {gauss(3.6,0.9,0.8)} \closedcycle;
  \addplot+[opacity=0.7,very thick,fill=red!30, draw=none, domain=0:2.9]
  {gauss(3.6,0.9,0.8)} \closedcycle;
  \addplot+[opacity=0.55,very thick,fill=red!50, draw=red!50!black, domain=2.9:4.3] {gauss(3.6,0.9,0.8)} \closedcycle;
\draw [color=red!66](axis cs:5.1,0.05) edge[implies] (axis cs:4.3,0.05);
\draw [color=red!66](axis cs:2.1,0.05) edge[implies] (axis cs:2.9,0.05);
\end{axis}
\end{tikzpicture}
\caption{Illustration of the mean cross lemma for $\tW_1$ in the special case that $p_1$ and $p_2$ have the same mean. If $\tW_1(p_1,p_2)$ is small, we can push the $\epsilon$-tails of $p_2$  to two points on the boundary of the new distribution to create a friendly perturbation 
$r_{p_2}$ that guarantees convex ordering.}
\label{fig.mean_cross_w1}
\end{figure}


\begin{lemma}
\label{lem:tw1_cross_mean}
Consider two distributions $p,q$ on the real line such that $\tW_1(p, q) \leq \epsilon$.
Then, for $g(x) = x$ or $g(x) = |x|$, one can find $r_p\in \mathbb{F}(p, 7\epsilon, W_1, g(x))$ and $r_q \in \mathbb{F}(q, 7\epsilon, W_1, g(x))$ 
such that $r_p$ is less than $r_q$ in the convex order with respect to the random variable $g(X)$:
$r_p \leq_{\mathrm{cx}} r_q$. This 
is equivalent to saying that for all convex functions $f$ such that the expectations exist, 
\begin{equation}
\mathbb{E}_{r_p}[f(g(X))] \leq \mathbb{E}_{r_q}[f(g(X))].
\end{equation}
\end{lemma}
The proof is deferred to Appendix~\ref{proof.tw1_cross_mean}. The idea is illustrated in Figure~\ref{fig.mean_cross_w1} in the special case that $p$ and $q$ have equal means. Intuitively, one can guarantee convex ordering by squeezing one of the distributions towards the mean. 
To apply the one-dimensional mean cross lemma, we consider all one-dimensional projections and identify the optimal direction.




The reason we only consider $g(x)$ instead of $f(x)$ in the friendly perturbation constraint is that the landscape of $f(x)$ can be complicated and it is harder to characterize the moving towards mean operation under $f(x)$. Thus for instance for 
second moment estimation, we consider friendly perturbations $r\in\mathbb{F}(p, \eta, W_1, |v^\top x|)$ instead of $r\in\mathbb{F}(p, \eta, W_1, |v^\top x|^2)$. As discussed in Example~\ref{example.psi_w1_resilience}, the sufficient condition and modulus of continuity remain unchange from this modification. 

We combine these observations to guarantee finite-sample robustness for the projection algorithm $q = \Pi(\hat p_n; \tW_1, \GG^{W_1}_\mathsf{sec})$, where $\GG^{W_1}_\mathsf{sec}$ is defined as
\begin{align}
    \GG^{W_1}_{\mathsf{sec}}(\rho, \eta) = \{p \mid \sup_{ \|v\|_2 = 1, r\in \mathbb{F}(p, \eta, W_1, |v^{\top}X|)} |\bE_{p}[|v^{\top}X|^2] - \bE_{r}[|v^{\top}X|^2]| \leq \rho  \}.
\end{align}


\begin{theorem}[Second moment estimation in Example~\ref{example.psi_w1_resilience}, $\tW_1$ projection]\label{thm.sec_tw_1_proj}
Assume $p^*$ has bounded $k$-th moment for $k>2$, i.e. 
    $\sup_{v\in\bR^d, \|v\|_2=1}\bE_{p^*}[|v^\top X|^k] \leq \sigma^k$
for some $\sigma>0$.
Denote $ \tilde \epsilon = \frac{C_1}{\delta} \left(\epsilon +  \sigma \sqrt{\frac{d}{n}}+\frac{\sigma }{\sqrt{n^{1-1/k}}}\right)$, where $C_1$ is some universal constant. 
Take the projection set as $ \GG = \GG_{\mathsf{sec}}^{W_1}(\max(4(7\tilde \epsilon)^2 + 14\sigma \tilde \epsilon, 14\sigma^{1+1/(k-1)}\tilde \epsilon^{1-1/(k-1)}), 7\tilde \epsilon)$, where $\GG_{\mathsf{sec}}^{W_1} $ is defined in Example~\ref{example.psi_w1_resilience}.
Then the projection algorithm $q = \Pi(\hat p_n; \tW_1, \GG)$ or $q = \Pi(\hat p_n; \tW_1, \GG, \tilde \epsilon/2)$    satisfies
\begin{align}
    \|\bE_{q}[XX^{\top}] - \bE_{p^*}[XX^{\top}]\|_2 \leq \min(\sigma^2, C_2 \sigma^{1+1/(k-1)}\tilde \epsilon^{1-1/(k-1)})
\end{align}
with probability at least $1-\delta$, 
where $C_2$ is some universal constant.
\end{theorem}


\begin{proof}
First, we show that the projected distribution $q$ is close to $p^*$ in $\tW_1$.  We know from Lemma~\ref{lem.tW_1_empirical_to_population} that under appropriate choice of $C_1$, with probability at least $1-\delta$, we have
\begin{align}
    \tW_1(p^*, \hat p_n) \leq \frac{\tilde \epsilon} {2}=  \frac{C_1}{\delta} \left(\epsilon +  \sigma \sqrt{\frac{d}{n}}+\frac{\sigma }{\sqrt{n^{1-1/k}}}\right).
\end{align}

Note that $\tW_1$ satisfies triangle inequality and $\mathcal{U}' \subset \mathcal{U}$. Therefore 
\begin{align}
    \tW_1(q, p^*) & \leq \tW_1(q, \hat p_n) + \tW_1(\hat p_n, p^*) \leq \tilde \epsilon.
\end{align}

From Lemma~\ref{lemma.population_limit} we know that the final result can be upper bounded by the modulus of continuity, thus it suffices to bound the term $\sup_{p_1, p_2\in \GG, \tW_1(p_1, p_2)\leq \tilde \epsilon} \|M_{p_1} - M_{p_2}\|_2 $.
We apply Lemma~\ref{lem:tw1_cross_mean} to show that the modulus of continuity can be bounded.
By symmetry, without loss of generality we can take some $v^*\in\bR^d, \|v^*\|_2=1$, such that
\begin{align}
    v^{*\top}(M_{p_1} -M_{p_2} )v^{*} = \|M_{p_1} -M_{p_2} \|_2.
\end{align}

From $p_1, p_2\in\GG^{W_1}(\rho_1(7\tilde \epsilon), \rho_2(7\tilde \epsilon), 7\tilde \epsilon)$ and $\tW_1(p_1, p_2)\leq  \tilde \epsilon$ and Lemma~\ref{lem:tw1_cross_mean}, we know that  there exist an $r_{p_1}\in \mathbb{F}(p_1, 7\tilde \epsilon, W_1, |v^{*\top} X|)$ and an $r_{p_2} \in \mathbb{F}(p_2,  7\tilde \epsilon, W_1, |v^{*\top} X|)$ such that
    \begin{align}
        \bE_{r_{p_1}}[(v^{*\top} X)^2 ] \leq \bE_{r_{p_2}} [(v^{*\top} X)^2].
    \end{align}
    
 From $p_1, p_2 \in \GG^{W_1}_\downarrow$, we know that 
    \begin{align}
        \bE_{{p_1}}[(v^{*\top} X)^2 ] - \bE_{r_{p_1}}[(v^{*\top} X)^2 ] \leq \max(4(7\tilde \epsilon)^2 + 14\sigma \tilde \epsilon, 14\sigma^{1+1/(k-1)}\tilde \epsilon^{1-1/(k-1)}), \\
        \bE_{r_{p_2}}[(v^{*\top} X)^2 ] - \bE_{{p_2}}[(v^{*\top} X)^2 ] \leq \max(4(7\tilde \epsilon)^2 + 14\sigma \tilde \epsilon, 14\sigma^{1+1/(k-1)}\tilde \epsilon^{1-1/(k-1)}).
    \end{align}
for all friendly perturbations $r_{p_1}$, $r_{p_2}$ of $p_1$, $p_2$.
Thus we know that
\begin{align}
      \|M_{p_1} -M_{p_2} \|_2 = &  v^{*\top}(M_{p_1} -M_{p_2} )v^{*}  \nonumber \\
       = &\bE_{p_1}[(v^{*\top}X)^2] -  \bE_{p_2}[(v^{*\top}X)^2] \nonumber \\
       =& \bE_{p_1}[(v^{*\top}X)^2] -  \bE_{r_{p_1}}[(v^{*\top}X)^2] + \bE_{r_{p_1}}[(v^{*\top}X)^2] -  \bE_{r_{p_2}}[(v^{*\top}X)^2] \nonumber \\
      & + \bE_{r_{p_2}}[(v^{*\top}X)^2] -  \bE_{{p_2}}[(v^{*\top}X)^2] \nonumber \\
      \leq & 2\max(4(7\tilde \epsilon)^2 + 14\sigma \tilde \epsilon, 14\sigma^{1+1/(k-1)}\tilde \epsilon^{1-1/(k-1)}).
\end{align}
This gives the desired result. 
\end{proof}





\paragraph*{Comparison and Interpretation}


When the third moment of $X$ is bounded by ${\sigma}^{3}$, the projection algorithm guarantees error
$O(\sigma^{3/2}\sqrt{\epsilon})$ for $\epsilon$ sufficiently small and $n\gtrsim \max(d/\epsilon^2, 1/\epsilon^4)$, while the same condition in $\TV$ perturbation would give error of $O(\sigma \epsilon^{2/3})$ for $n\gtrsim d/\epsilon^2$ (Theorem~\ref{thm.tTV_joint_correct}).


\subsection{$\tW_1$ projection for Linear Regression}


A close inspection of the proof of Theorem~\ref{thm.sec_tw_1_proj} shows that it can be generalized to any loss $L$ such that $\sF_\theta$ contains only functions of the form $f(|v^\top x|)$, where all the $f$ are convex functions
(see Proposition~\ref{prop.tW1_general} for proof). We then obtain the following result for robust linear regression under $W_1$ perturbation:

\begin{theorem}[Linear regression in Example~\ref{example.linreg_w1_bounded}, $\tW_1$ projection]
\label{thm.linreg_tw_1_proj}


Denote by $X' = [X, Z]$ the $d+1$ dimensional vector. Assume that $\|\theta\|_2\leq R$ and  $p^*$ satisfies:
\begin{align}
   \sup_{v\in\bR^{d+1}, \|v\|_2=1}  \bE_{p^*}\bigg[{|v^{\top}X'|^{k}}\bigg] \leq \sigma_1^{k}, 
   \bE_{p^*}[Z^2] \leq \sigma_2^2.
\end{align} 
Here $k> 2$. 
Denote $\bar R = \max(R, 1)$, $ \tilde \epsilon = \frac{C_1}{\delta} \left(\epsilon + \sigma_1  \bar R\sqrt{ d/n}+ \sigma_1 \bar R/\sqrt{n^{1-1/k}}\right)$,  where $C_1$ is some universal constant. For $\GG$ in Example~\ref{example.linreg_w1_bounded} with appropriate parameters, the projection algorithm $q = \Pi(\hat p_n; \tW_1, \GG)$ or $q = \Pi(\hat p_n; \tW_1, \GG,  \tilde \epsilon/2)$ satisfies
\begin{align}
    \bE_{p^*}[(Y-X^\top \theta^*(q))^2 ] \leq \sigma_2^2 + C_2 \bar R^2 (\sigma_1^{1+1/(k-1)} (\bar R \tilde \epsilon)^{1-1/(k-1)} + (\bar R \tilde \epsilon)^2)
\end{align} 
with probability at least $1-\delta$, where $C_2$ is some universal constant. 
\end{theorem}

The proof is the same as Theorem~\ref{thm.sec_tw_1_proj} for second moment estimation, except that in Lemma~\ref{lem.tW_1_empirical_to_population}, we use $\sup_{v\in\bR^{d+1}, \|v\|_2=1}\bE_{p^*}[|v^\top X''|^k] \leq \bar R^k\sigma_1^k$ for $X'' = [X, Y]$. 

\paragraph*{Interpretation}

Taking $k=3$,  the projection algorithm guarantees predictive loss $\sigma^2 + O_{\sigma_1, \sigma_2, \bar R}(\sqrt{\epsilon})$ for $\epsilon$ sufficiently small and $n\gtrsim \max(d/\epsilon^2, 1/\epsilon^4)$.


\subsection{Expanding the set for second moment estimation}

Similar to Section~\ref{sec.expand}, we implement the expanding set idea to provide both statistically efficient and computationally efficient algorithm via $W_1$ projection algorithm.

\begin{theorem}[Second moment estimation in Example~\ref{example.psi_w1_resilience}, $W_1$ or $\tW_1$ projection]\label{thm.efficient_sec_w1}
Assume that $p^*$ has bounded $k$-th moment for $k>2$, i.e. 
    $\sup_{v\in\bR^d, \|v\|_2=1}\bE_{p^*}[|v^\top X|^k] \leq \sigma^k$
for some $\sigma>0$, and that the adversary is able to corrupt the true empirical distribution $\hat p_n^*$ to some distribution $\hat p$ such that $W_1(\hat p_n^*, \hat p)\leq \epsilon$. 
Take the projection set as $ \GG = \{p \mid \sup_{v\in\bR^d, \|v\|_2=1}\bE_{p}[|v^\top X|^k] \leq 2\sigma^k\}$. When $n\gtrsim (d\log(d/\delta))^{k/2}$ the projection algorithm $q = \Pi(\hat p_n; W_1 / \tW_1, \GG)$ or $q = \Pi(\hat p_n; W_1 / \tW_1, \GG, \epsilon)$    satisfies
\begin{align*}
    \|\bE_{q}[XX^{\top}] - \bE_{p^*}[XX^{\top}]\|_2 \leq \min(\sigma^2, C_1 \sigma^{1+1/(k-1)}  \epsilon^{1-1/(k-1)})+C_2\sigma^2 \max(\sqrt{\frac{ d\log(d/\delta)}{n\delta^{2/k}}},  \frac{ d\log(d/\delta)}{n\delta^{2/k}}).
\end{align*}
with probability at least $1-\delta$, 
where $C_1, C_2$ are some universal constants.
\end{theorem}
The proof is deferred to Appendix~\ref{proof.efficient_sec_w1}. 
When $k=4$, we would like to solve the following constrained optimization problem:
\begin{align*}
   &  \min_{y_1,\cdots, y_n} \frac{1}{n}\sum_{i=1}^n \|x_i - y_i\|_2 \nonumber \\ 
     \text{subject to} & \sup_{v\in\bR^d} \frac{1}{n}\sum_{i=1}^n  (v^\top y_i)^4\leq 2\sigma^4.
\end{align*}
The algorithm can be relaxed and made efficient via sum-of-squares program by assuming that the $k$-th moment bound on distribution is certifiable. 

==> temp.tex <==
As a starting point we consider the case of robust mean estimation under $\TV$ corruption, where  $L(p^*, \theta) = \|\theta - \bE_{p^*}[X]\|_2$. We define $\GG$ based on the notion of \emph{resilient distributions} 
introduced in \citet{steinhardt2018resilience} (implicit in~\cite{diakonikolas2017being}).  A distribution $p$ over $\bR^d$ is $(\rho, \epsilon)$-resilient if 
\begin{equation}
\label{eq.resilience_mean_intro}
\|\bE_{p}[X \mid E] - \bE_{ p}[X]\|_2 \leq \rho \text{ for all events $E$ with } \bP_p(E) \geq 1-\epsilon.
\end{equation}
This says that all ``$\epsilon$-deletions'' of $p$ must have a mean similar to the mean of $p$. This property holds, for instance, 
for sub-Gaussians (with $\rho \asymp \epsilon \sqrt{\log(1/\epsilon)}$) as well as
distributions with bounded covariance (with $\rho \asymp \sqrt{\epsilon}$). This also includes 
sub-exponential distributions (with $\rho \asymp \epsilon \log(1/\epsilon)$) and distributions with bounded 
$k$-th moments (with $\rho \asymp \epsilon^{1-1/k}$). Importantly, $\rho$ usually has no 
explicit dependence on the dimension $d$. 


Let $\Gmean(\rho, \epsilon)$ denote the family of $(\rho, \epsilon)$-resilient distributions.  Then the modulus satisfies $\modu(\Gmean(\rho,\epsilon), \epsilon) \leq 2\rho$. 
The reason for this is a \emph{midpoint property} of $\TV$ 
distance (Lemma~\ref{lem.G_TV_mean_modulus}, implicit in~\citet{diakonikolas2016robust, diakonikolas2017being, steinhardt2017certified}) : if $\TV(p_1, p_2) \leq \epsilon$ then there is a midpoint $r$ that can be obtained from either of the $p_i$ 
by conditioning on an event of probability $1-\epsilon$. Thus $\bE_r[X]$ is close to both $\bE_{p_1}[X]$ and $\bE_{p_2}[X]$ by
resilience, and so $\bE_{p_1}[X]$ and $\bE_{p_2}[X]$ are close by the triangle inequality.  
The modulus guarantees optimal worst-case loss in population for all the concrete cases above. We discuss these results in detail in   Example~\ref{example.mean_psi} and Section~\ref{sec.mean_estimation_G}.



Before diving into the finite-sample analysis, we motivate our design in the population setting, where the sample size $n = \infty$. 
We consider the population MD functional in~\eqref{eq.mdfintro} that takes the form 
\begin{equation}\label{eq.population_mdfintro}
\hat{\theta}(p) = \theta^*(q), \text{ where } q = \argmin_{q \in \GG} D(q, p).
\end{equation}
The worst-case loss of the MD functional $\hat{\theta}(p)$ is upper bounded by the \emph{modulus of continuity}~\cite{donoho1988automatic}, defined as
\begin{equation}
\modu(\GG, 2\epsilon) = \sup_{p_1, p_2 \in \GG : D(p_1, p_2) \leq 2\epsilon} L(p_1, \theta^*(p_2)).
\end{equation}
 When we know the corruption level $\epsilon$ explicitly, it suffices to find some $q\in\GG$ that is within $\epsilon$-ball of $p$ instead of doing projection to achieve the same bound.  
To bound the worst-case loss and the performance of MD functional estimator, we mainly focus on bounding the modulus of $\mathcal{G}$. %



We want a way of measuring the tails of a distribution. We do so using \emph{Orlicz norms}:

\begin{definition}[Orlicz function and norm]\label{def.orlicz_function}
A function $\psi: [0, +\infty) \mapsto [0, +\infty)$ is called an \emph{Orlicz function} if $\psi$ is convex, non-decreasing, and satisfies $\psi(0) = 0$, $\psi(x) \to \infty$ as $x\to \infty$. For a given Orlicz function $\psi$, the Orlicz norm of a random variable $X$ is defined as
\begin{align}
    \| X \|_{\psi} \triangleq \inf\left \{ t>0 : \bE_p\left [\psi\left(|X|/t\right )\right ] \leq 1\right \}.
\end{align}
\end{definition}
As special cases, we say that a random variable $X \sim p$ is \emph{sub-Gaussian} with parameter $\sigma$ if 
$\|\langle X - \bE_p[X], v \rangle\|_{\psi_2} \leq \sigma$ whenever $\|v\|_2 \leq 1$, where $\psi_2(x) = e^{x^2}-1$.
We define a \emph{sub-exponential} random variable similarly for the function $\psi_1(x) = e^x-1$.






\subsection{Warm-up: Mean Estimation}\label{sec.mean_estimation_G}

As a warm-up, we consider the 
special case of mean estimation with cost function $L(p, \theta) = \|\theta - \bE_p[X]\|$ for some norm $\|\cdot\|$. 
\citet{steinhardt2018resilience} introduced 
the set of \emph{resilient} distributions which exactly satisfy the above properties and will be our 
starting point for more general settings (also implicit in~\cite{diakonikolas2017being}). 
A distribution is called \emph{resilient} if every $(1-\eta)$-subset of the distribution 
has a similar mean. 
More formally, the set of resilient distributions with parameters $(\rho, \eta)$ are
\begin{align} \label{eqn.oldresilience}
    \GG_{\mathsf{mean}}(\rho, \eta) \eqdef \big\{p  \mid \|\bE_r[X] - \bE_p[X] \| \leq \rho \text{ for all } r \leq \frac{p}{1-\eta}\big\},
\end{align}
where $\|\cdot\|$ is an arbitrary norm. 
The inequality $r\leq \frac{p}{1-\eta}$ can be formally understood as $\frac{dr}{dp}\leq \frac{1}{1-\eta}$, where $\frac{dr}{dp}$ is the Radon-Nikodym derivative; an equivalent characterization is that 
$r$ can be obtained from $p$ by conditioning on an event $E$ of probability at least $1-\eta$, which is shown in Lemma~\ref{lem.deletionrproperties}.
Thus $r$ can be thought of as an ``$\eta$-deletion'' of $p$.

The modulus of continuity $\modu$ of $\Gmean$ is upper bounded by $2\rho$.  
The key idea is that any two distributions that are close in $\TV$ have a \emph{mid-point} distribution that is a deletion of both 
distributions (Lemma~\ref{lem.deletionrproperties}). The mid-point distribution has mean close to both distributions via resilience, 
and it follows from the triangle inequality that the modulus of $\GG_{\mathsf{mean}}$ is bounded. 
The idea of mid-point is also used implicitly in~\citet{steinhardt2017certified, diakonikolas2016robust, diakonikolas2017being}.



\subsubsection*{Not too small: Concrete examples for $\GG$ }
Since the definition of $\GG$ is abstract, we provide below sufficient conditions for inclusion in $\GG$ in 
the case of linear regression,
joint estimation of mean and covariance under the transformed space and
second moment estimation. 
In these cases $\GG$ subsumes many known distribution families in the robust statistics literature, 
while at the same time Theorem~\ref{thm.G_fundamental_limit} provides a bound 
on the population limit that matches or improves on known results.





\begin{figure}[!htbp]
\centering
\begin{tikzpicture}
    \draw [opacity=1, very thick, fill=red!50, draw= red!50!black](2.4, 0.0) {ellipse (2cm and 1cm)};
     \draw [opacity=0.6,  very thick, fill= cyan!20, draw= cyan!20!black](2.0, 1.0) {ellipse (3cm and 2.5cm)};
      \draw [opacity=0.4, fill= yellow!20, draw= yellow!20!black](2.5, 1.5) {ellipse (4.5cm and 3.2 cm)};
     \draw  [](3.3, -0.5) node {$p^*\in\GG$};
     \draw  [](1.3, 0) node {\Large $\GG$};
     \draw  [](0.3, 1.8) node {\Large $\GG'$};
     \draw  [](-0.6, 3.5) node {\Large $\cM$};
       \draw [radius=1.5pt,fill](3.4, -0.23) circle;
     \draw  [](3.35, 2.42) node {$\hat p'\in\GG'$};
      \draw [radius=1.5pt,fill](3.5,2.85) circle;
     \draw  [](2.6,5.2) node {$\hat p_n^*$};
      \draw [radius=1.5pt,fill](2.8, 4.85) circle;
    \draw  [](4.51, 4.67) node {$q\in\cM$};
      \draw [radius=1.5pt,fill](4.5,4.3) circle;
     \draw  [](9,4.5) node {Observed distribution $\hat p_n$};
      \draw [radius=1.5pt,fill] (7.2, 4.0) circle;
    \draw (7.2, 4.0) edge[->] node[below, rotate=48,yshift=-1.5]{{\scriptsize $ \tTV_\mathcal{H}\lesssim \epsilon + \sqrt{\mathsf{vc}(\mathcal{H})/n}$, $\TV$ large}} (3.4, -0.23);
    \draw (7.2, 4.0) edge[->] node[above, rotate=16, xshift=-0.5]{{\scriptsize $\tTV_\sH\leq  \TV\lesssim \epsilon + 1/n$}} (3.5,2.85); 
    \draw (7.2, 4.0) edge[->] node[above, rotate=-8]{{\scriptsize projection}} (4.56,4.3);
     \draw (2.8, 4.85) edge[->] node[below, rotate=-70]{{\scriptsize $\TV$ small}} (3.45,2.9);
\end{tikzpicture}
\caption{
Illustration of projection algorithm. By perturbing $\hat p_n^*$ to $\hat p'$ a small amount ($\TV(\hat p_n^*, \hat p')\lesssim \epsilon + 1/n$) under $\TV$, we can ensure $\hat p' \in \GG'$ and control $\TV(\hat p_n, \hat p')$ simultaneously. Thus projecting $\hat p_n$ onto a larger set $\cM$ can guarantee $ \tTV_\sH(q, \hat p_n)\leq \TV(q, \hat p_n)\lesssim \epsilon+1/n$. In contrast, projecting onto the original $\GG$ (as Section~\ref{sec.finite_sample_algorithm_weaken}) can only guarantee $\tTV_\mathcal{H}(q, \hat p_n)\lesssim \epsilon+\sqrt{\mathsf{vc}(\mathcal{H})/n}$, which gives sub-optimal sample complexity in many cases.}
\label{fig.projection_illustration}
\end{figure}



\subsubsection*{Union bound}
Our first observation is that even if $\GG$ is small, we can take $\MM$ to be the family of resilient 
distributions while maintaining similarly small modulus. 
Thus we only need $\hat{p}_n^*$ to be {resilient},
which is easier to satisfy than e.g.~bounded moments or sub-Gaussianity.
For distributions with moment generating functions, a union bound leads to the following typical result~(Lemma~\ref{lem.subgaussian_empirical_resilience}): if $p^*$ is sub-Gaussian with parameter $\sigma$, then for any fixed $\eta$, the empirical distribution $\hat p_n^*$ 
is $(\rho, \eta)$-resilient with probability $1-\delta$, for $\rho = O(\sigma (\sqrt{\eta \frac{d+\log(1/\delta)}{n}} + \eta \sqrt{\log(1/\eta)}))$, which gives tighter bound for resilience paramter than~\citet[Lemma  4.4]{diakonikolas2019robust}. 
We thus obtain:
\begin{theorem}[Sub-Gaussian]\label{thm.general_subgaussian_tv_projection}
Denote $\tilde \epsilon = 2(\sqrt{\epsilon} + \sqrt{\frac{\log(1/\delta)}{2n}})^2$.
There exist some constants $C_1, C_2$ such that the following statement is true. Take $\GG$ as family of sub-Gaussian with parameter $\sigma$ and $\cM$ as resilient set, i.e.
\begin{align}
    \GG & =  \bigg\{ p \mid \sup_{v\in\bR^d, \|v\|_2=1} \bE_p\bigg[\exp\bigg(\left( \frac{|v^{\top}(X-\bE_p[X])|}{\sigma}\right)^2\bigg) \bigg] \leq  2 \bigg\},\\
  \cM & = \GG_{\mathsf{mean}}\bigg( C_1\sigma\cdot \bigg(\epsilon \sqrt{\log(1/\epsilon)} + \sqrt{ \frac{d+\log(1/\delta)}{n}}\bigg) , \tilde \epsilon \bigg),
\end{align}
where $\GG_{\mathsf{mean}}$ is defined in~\eqref{eqn.oldresilience}.  If $p^*\in\GG$ and $\tilde \epsilon\leq 1/2$,
then the projection $q = \Pi(\hat p_n; \TV / \tTV_\mathcal{H}, \cM)$ of $\hat{p}_n$ onto $\MM$ satisfies:
\begin{align}
 \|\bE_{p^*}[X]- \bE_q[X] \|_2 & \leq   C_2\sigma \cdot \bigg(\epsilon \sqrt{\log(1/\epsilon)} + \sqrt{\frac{d+\log(1/\delta)}{n}} \bigg)
\end{align}
 with probability at least $1-3\delta$. Moreover, 
this bound holds for any $q \in \MM$ within $\TV$ (or $\tTV$) distance $\tilde \eps/2$ of $\hat{p}_n$.

\end{theorem}
The proof is deferred to Appendix~\ref{proof.general_subgaussian_tv_projection}. 


\subsection{Proof of Theorem~\ref{thm.general_subgaussian_tv_projection}}\label{proof.general_subgaussian_tv_projection}


\begin{proof}
We verify the five conditions in Theorem~\ref{thm.admissible-2}. 

\begin{enumerate}
    \item \textbf{Robust to perturbation:} True since $\TV$ satisfies triangle inequality.
    \item \textbf{Limited Corruption:} It follows from Lemma~\ref{lem.coupling_TV} that  with probability at least $1-\delta$, 
    \begin{align}
        \TV(\hat p_n, \hat p_n^*)\leq \left(\sqrt{\epsilon} + \sqrt{\frac{\log(1/\delta)}{2n}}\right)^2 = \frac{\tilde\epsilon}{2}.
    \end{align}
\item \textbf{Set for (perturbed) empirical distribution:} It can be seen from Lemma~\ref{lem.subgaussian_empirical_resilience}  that for some fixed $\eta\in[0, 1/2]$, with probability at least $1-\delta$,  there exists some constant $C$ such that
\begin{align}
  \hat p_n^* \in   \GG_{\mathsf{mean}}\left( C \sigma \cdot \left( \sqrt{\frac{d + \log(1/\delta)}{n}} +  \eta \sqrt{\log(1/\eta)} \right), \eta \right).
\end{align}

 
\item \textbf{Generalized Modulus of Continuity:}

 We construct
$\cM  = \GG'=  \GG_{\mathsf{mean}}\left(C\sigma \cdot \left(  \sqrt{\frac{d + \log(1/\delta)}{n}} +  \tilde{\epsilon} \sqrt{\log(1/\tilde{\epsilon})} \right), \tilde{\epsilon}\right)$. Thus it follows from the population limit of $\GG_{\mathsf{mean}}$ in Lemma~\ref{lem.G_TV_mean_modulus} that for some constant $C_1$, we have
\begin{align}\nonumber
    \sup_{p_1^*\in \mathcal{M}, p_2^* \in \GG', \TV(p_1^*, p_2^*)\leq \tilde \epsilon} \|\bE_{p_1^*}[X]-\bE_{p_2^*}[X]\|_2 & \leq   C_1\sigma\left(\sqrt{\frac{d+\log(1/\delta)}{n}} + \tilde{\epsilon} \sqrt{\log(1/\tilde{\epsilon})}\right).
\end{align}
Since $f(x) = x\sqrt{\log(1/x)}$ is a concave function, and $f(0)=0$, we have 
\begin{align}
    f(a+b) = \frac{a}{a+b}f(a+b) + \frac{b}{a+b}f(a+b) \leq f(a)+f(b).
\end{align}
From the assumption in theorem statement we know that  $n \geq \log(1/\delta)$, we have
\begin{align}\label{eqn.concave_upper_bound}
    \tilde{\epsilon} \sqrt{\log(1/\tilde{\epsilon})} \lesssim {\epsilon} \sqrt{\log(\frac{1}{\epsilon})} + \frac{\log(1/\delta)}{n}\sqrt{\log(\frac{n}{\log(1/\delta)})} \lesssim {\epsilon} \sqrt{\log(\frac{1}{\epsilon})} + \sqrt{\frac{\log(1/\delta)}{n}}.
\end{align}
From Theorem~\ref{thm.tTV_mean}, we know that the generalized modulus for $\tTV_\mathcal{H}$ is the same as $\TV$ for resilient set.
\item \textbf{Generalization bound:} Since we take $\hat p' = \hat p_n^*$, we have
\begin{align}
    \|\bE_{p^*}[X]- \bE_q[X] \|_2 \leq  \|\bE_{p^*}[X]- \bE_{\hat p_n^*}[X] \|_2 +   \|\bE_{\hat p_n^*}[X] - \bE_{q}[X]\|_2 .
\end{align}
Thus by with probability at least $1-\delta$, 
\begin{align}
        \|\bE_{p^*}[X]- \bE_q[X] \|_2 \leq \|\bE_{\hat p_n^*}[X] - \bE_{q}[X]\|_2  + C\sigma\sqrt{\frac{d+\log(1/\delta)}{n}}.
\end{align}
The convergence of $\|\bE_{\hat p_n^*}[X] - \bE_{p^*}[X]\|_2  $ is from~\citep[Equation (5.5)]{lugosi2017lectures}.
\end{enumerate}







Combining the five conditions, from Theorem~\ref{thm.admissible-2}, for projection algorithm $q = \argmin\{\TV(q, \hat p_n) \mid q \in \cM\}$, we have with probability at least $1-3\delta$,
\begin{align}
 \|\bE_{p^*}[X]- \bE_q[X] \|_2 & \leq C\sigma \cdot \left(\sqrt{\frac{d+\log(1/\delta)}{n}} + \epsilon\sqrt{\log(1/\epsilon)}\right),
\end{align}
where $C$ is some universal constant.
\end{proof}




\begin{example}[Second moment estimation]\label{example.G_TV_sec1}
Take $B(p, M) = \|I - M^{-1/2}M_pM^{-1/2} \|_F$,  $L(p,M) = \|I - M_p^{-1/2}MM_p^{-1/2}\|_F$ as above.
For a random variable $X \sim p$ with second moment $M_p$, let $Y = M_p^{-1/2}X$. 
Assume that $Y$ satisfies
\begin{align}
\label{eq.cov_mahalanobis_tv}
\sup_{U \in\bR^{d\times d}, \|U\|_F = 1}
\bE_{p}\left [\psi \left (\frac{|Y^{\top}UY-\bE_p[Y^{\top}UY]|}{\kappa}\right )\right ] \leq 1.
\end{align}
Then $p \in \GG(\rho, 2\rho(1+\rho), \eta)$ for $\rho = 4\kappa\eta \psi^{-1}(1/\eta)$ when $\eta \in [0, \frac{1}{2}]$ and $\rho(1+\rho) < \frac{1}{2}$.
Thus the population limit for the set is 
$\Theta(\kappa\epsilon\psi^{-1}(\frac{1}{\epsilon}))$ when the perturbation level is $\epsilon \leq \frac{\eta}{2}$.

\end{example}

\begin{proof}

We first show that $p\in \GG_{\downarrow}^{\TV}$. Note that the condition in $\GG_{\downarrow}^{\TV}$ can be written as
\begin{align}
    \sup_{r\leq \frac{p}{1-\eta}} \|\bE_p[M_p^{-1/2}XX^{\top}M_p^{-1/2}] - \bE_r[M_p^{-1/2}XX^{\top}M_p^{-1/2}] \|_F\leq \rho.
\end{align}
Recall that we define $Y =M_p^{-1/2} X$. We flatten $YY^T$ as a vector $Y^{\otimes 2}$.
Then $p\in \GG_\downarrow$ is equivalent to requiring that the distribution of $Y^{\otimes 2}$ is inside set $\GG_{\mathsf{mean}}$. 
By  Lemma~\ref{lem.cvx_mean_resilience}, we know that from the given assumption in \eqref{eq.cov_mahalanobis_tv},   the distribution of $Y^{\otimes 2}$ is inside $\GG_{\mathsf{mean}}(4\kappa\eta\psi^{-1}(\frac{1}{\eta}), \eta)$ for all $\eta \in [0, 1/2)$,  we know that the LHS of above equation can be controlled with $\rho = 4\kappa\epsilon\psi^{-1}(\frac{1}{\epsilon})$. 

Now we validate that $\GG_{\downarrow}^{\TV}(\rho, \eta) \subset \GG_{\uparrow}^{\TV}(2\rho(1+\rho), \eta)$. By $p\in\GG_{\downarrow}$ and the condition in $\GG_{\uparrow}$, we have 
\begin{align}
    \|I - M_p^{-1/2}M_rM_p^{-1/2} \|_F  & \leq \rho, \\
    \|I - M^{-1/2}M_r M^{-1/2} \|_F  & \leq \rho 
\end{align}
From the first bound, we know that $ \|M_p^{-1/2}M_r^{1/2} \|_2^2 \leq 1 + \rho$.
We  bound the term:
\begin{align}
    \|I - M_p^{-1/2}M M_p^{-1/2} \|_F & = \|M_p^{-1/2}M_r^{1/2}(M_r^{-1/2}M_pM_r^{-1/2} - M_r^{-1/2}M M_r^{-1/2}  )M_r^{1/2}M_p^{-1/2} \|_F \nonumber \\
    & \leq \|M_p^{-1/2}M_r^{1/2} \|_2^2 \| M_r^{-1/2}M_pM_r^{-1/2} - M_r^{-1/2}M M_r^{-1/2}  \|_F \nonumber \\
    & \leq \|M_p^{-1/2}M_r^{1/2} \|_2^2 \bigg( \|I -  M_r^{-1/2}M_pM_r^{-1/2} \|_F + \| I - M_r^{-1/2}M M_r^{-1/2}  \|_F \bigg)\nonumber \\
    & \leq  2\rho (1+\rho).
\end{align}
It can be seen from Theorem~\ref{thm.G_fundamental_limit} that when the perturbation level is $\epsilon$, the population limit for this set  is upper bounded by $8\kappa \epsilon\psi^{-1}(\frac{1}{2\epsilon}) \big(1+4\kappa\epsilon\psi^{-1}(\frac{1}{2\epsilon})\big)$.

The lower bound on population limit can be seen from Lemma~\ref{lem.Wf_orlicz_lower_bound_limit}. 

\end{proof}
When $\psi(x) = x^2$ condition \eqref{eq.cov_mahalanobis_tv} asks that $YY^\top$ has bounded covariance when considered as a 
$d^2$-dimensional random variable. 

\paragraph*{Interpretation} 
The population limit for zero mean Gaussian distributions is $\Theta(\epsilon)$~\citep{diakonikolas2019robust}. By taking $\psi(x) = \exp(x)-1$, we generalize the Gaussian assumption to a larger non-parametric family with rate-optimal population limit $O(\epsilon \log(1/\epsilon))$, which matches the result in~\citet{diakonikolas2017being}.

Similar rate of $\epsilon \psi^{-1}(1/\epsilon)$ for population limit can also be derived if we take $L(p, M) = \|\bE_p[XX^\top] - M\|_2$ and assume $p$ satisfies
\begin{align}
    \sup_{v\in\bR^d, \|v\|_2\leq 1} \bE_p\left[\psi\left(\frac{(v^\top X)^2}{\sigma^2}\right)\right] \leq 1. 
\end{align}
This is a direct corollary of Lemma~\ref{lem.cvx_mean_resilience} (and Lemma~\ref{lem.centering_psi} for converting non-centered assumption to centered assumption). 




\subsubsection*{$\tTV_{\sH}$ projection for second moment estimation}
Let $M_p = \bE_p[XX^{\top}]$. 
For second moment estimation under the loss $L(p,M) = \|I - M_p^{-1/2}M M_p^{-1/2}\|_F$ in Example~\ref{example.G_TV_sec1}, we 
take $\sH$ to be
\begin{align}\label{eqn.H_sec_multiplicative}
    \mathcal{H} & = \{\mathsf{Tr}(A(I - M^{-1/2}XX^{\top}M^{-1/2})) \mid  \|A\|_F\leq 1, M \in \bR^{d\times d} \},
\end{align}
motivated by the dual representation
of $ B(p,M) = \|I - M^{-1/2}M_pM^{-1/2}\|_F$ as the Frobenius norm.


Directly applying mid-point lemma to $f\in\mathcal{H}$ cannot control the modulus since $B(p,M)$ does not satisfy triangle inequality.
Instead, we apply minimax theorem to control the modulus of continuity (general version Lemma~\ref{lemma.minimaxmodulus}). We show the theorem as below and defer the proof to Appendix~\ref{appendix.sec_tvt_proof}. 

\begin{theorem}\label{thm.secondmomenttvtilde}
Denote $\tilde \epsilon = 2\epsilon + 2 C^{\mathsf{vc}} \sqrt{\frac{d^2+1+\log(1/\delta)}{n}}$.  Assume $p^* \in \GG(\rho_1(\tilde \epsilon), \rho_2(\tilde \epsilon),  \tilde \epsilon))$ in Example~\ref{example.G_TV_sec1}. For $\mathcal{H}$ designed in (\ref{eqn.H_sec_multiplicative}), let $q$ denote the output of the projection algorithm $\Pi(\hat{p}_n; \tTV_{\mathcal{H}}, \GG)$. Then, with probability at least $1-\delta$, 
\begin{align}
    \|I  - M_q^{-1/2} M_{p^*}M_q^{-1/2} \|_F \leq \rho_2(\tilde \epsilon) = \rho_2\left (2\epsilon + 2 C^{\mathsf{vc}} \sqrt{\frac{d^2+1+\log(1/\delta)}{n}} \right ).
\end{align}
\end{theorem}



\subsubsection*{Interpretation and Comparison}

\citet{diakonikolas2017being} constructed an algorithm that achieves error $\epsilon \log(1/\epsilon)$ with constant probability given sample size $n \gtrsim \frac{d^2}{\epsilon^2} \mathrm{polylog}(d/\epsilon)$ when the real distribution is Gaussian. We achieve the same error for all resilient distributions given sample size $n\gtrsim \frac{d^2}{\epsilon^2}$.


In the finite-sample result, we need to slightly shrink the resilient set from 
$
    \GG^\TV_\downarrow(\rho_1(\tilde \epsilon), \tilde \epsilon)\cap \GG^\TV_\uparrow(\rho_1(\tilde \epsilon), \rho_2(\tilde \epsilon), \tilde \epsilon)
$
to 
$
    \GG^\TV_\downarrow(\rho_1(\tilde \epsilon), \tilde \epsilon)\cap \GG^\TV_\uparrow(2\rho_1(\tilde \epsilon), \rho_2(\tilde \epsilon), \tilde \epsilon).
$
The conditions in the first part of the theorem still imply that $p^*$ is inside this 
smaller set with appropriate parameters.
The shrinkage comes from the following consideration: 
when using the mid-point lemma, we can only find the mid-point for $p $ and $q$ under the same transform function $f(X)$  while the excess predictive loss in the original $\GG^\TV$ requires the mid-point for two different functions.

